The Lov\'asz Hinge: A Novel Convex Surrogate for Submodular Losses

Learning with non-modular losses is an important problem when sets of predictions are made simultaneously. The main tools for constructing convex surrogate loss functions for set prediction are margin rescaling and slack rescaling. In this work, we show that these strategies lead to tight convex surrogates iff the underlying loss function is increasing in the number of incorrect predictions. However, gradient or cutting-plane computation for these functions is NP-hard for non-supermodular loss functions. We propose instead a novel surrogate loss function for submodular losses, the Lov\'asz hinge, which leads to O(p log p) complexity with O(p) oracle accesses to the loss function to compute a gradient or cutting-plane. We prove that the Lov\'asz hinge is convex and yields an extension. As a result, we have developed the first tractable convex surrogates in the literature for submodular losses. We demonstrate the utility of this novel convex surrogate through several set prediction tasks, including on the PASCAL VOC and Microsoft COCO datasets.

==> Generalization.tex <==
\section{New Section on the generalization of Lov\'{a}sz Hinge}


==> IntroductionArXiv.tex <==
\section{Introduction}
Statistical learning has largely addressed problems in which a loss function decomposes over individual training samples.
However, there are many circumstances in which non-modular losses can lead to better end results.  This is the case when multiple outputs of a prediction system are used as the basis of a decision making process that leads to a single real-world outcome.  These dependencies in the effect of the predictions (rather than a statistical dependency between predictions themselves) are therefore properly incorporated into a learning system through a non-modular loss function.
In this paper, we aim to provide a theoretical and algorithmic foundation for a novel class of learning algorithms that make feasible learning with submodular losses, an important subclass of non-modular losses that is currently infeasible with existing algorithms.  This paper provides a unified and extended presentation of our conference paper~\cite{DBLP:conf/icml/YuB15}.  %We demonstrate that existing learning algorithms are suited to increasing loss functions, but they are NP-hard to optimize for non-supermodular losses.


Convex surrogate loss functions are central to the practical application of empirical risk minimization.  Straightforward principles have been developed for the design of convex surrogates for binary classification and regression~\cite{bjm-ccrb-05}, and in the structured output setting margin and slack rescaling are two principles for defining convex surrogates for more general output spaces~\cite{tsochantaridis2005large}.  Despite the apparent flexibility of margin and slack rescaling in their ability to bound arbitrary loss functions, there are fundamental limitations to our ability to apply these methods in practice: (i) they provide only loose upper bounds to certain loss functions, (ii) computing a gradient or cutting plane is NP-hard for submodular loss functions, and (iii) consistency results are lacking in general~\cite{citeulike:4464052,Tewari:2007}.  In practice, modular losses, such as Hamming loss, are often applied to maintain tractability, although non-modular losses, such as the Jaccard loss have been applied in the structured prediction setting~\cite{BlaschkoECCV2008,NowozinCVPR2014}.  We show in this paper that the Jaccard loss is in fact a submodular loss, and our proposed convex surrogate provides a polynomial-time tight upper bound.

\mycorr{Non-modular losses have been (implicitly) considered in the context of multilabel classification problems. 
\cite{cheng2010bayes} uses the Hamming loss and subset 0-1 loss which are modular, and a rank loss which is supermodular; \cite{petterson2011submodular} introduces submodular pairwise potentials, not submodular loss functions, while using a non-submodular loss based on F-score.
\cite{li2014condensed} uses (weighted) Hamming loss which is modular, but also proposes a new tree-based algorithm for training; \cite{doppa2014hc} uses modular losses e.g.\ Hamming loss and F1 loss  which is non-submodular.
However, non-supermodular loss functions are substantially more rare in the literature. % Two very interesting submodular functions are set cover and influence in networks. 
}
%(perhaps look at Nowozin CVPR 2014 paper introduction for some ideas about how to argue this point).

In this work, we introduce an alternate principle to construct convex surrogate loss functions for submodular losses based on the Lov\'{a}sz extension of a set function.  
\mycorr{
The Lov\'{a}sz extension of a submodular function is its convex closure, and has been used in other machine learning contexts e.g.~\cite{bach2010structured,iyer2013lovsz}.
}
We analyze the settings in which margin and slack rescaling are tight convex surrogates by finding necessary and sufficient conditions for the surrogate function to be an extension of a set function.  Although margin and slack rescaling generate extensions of \emph{some} submodular set functions, their optimization is NP-hard. 
We therefore propose a novel convex surrogate for submodular functions based on the Lov\'{a}sz extension, which we call the Lov\'{a}sz hinge.
In contrast to margin and slack rescaling, the Lov\'{a}sz hinge provides a tight convex surrogate to \emph{all} submodular loss functions, and computation of a gradient or cutting plane can be achieved in $\mathcal{O}(p \log p)$ time with a linear number of oracle accesses to the loss function.  We demonstrate empirically fast convergence of a cutting plane optimization strategy applied to the Lov\'{a}sz hinge, and show that optimization of a submodular loss results in lower average loss on the test set.

\iffalse
\begin{itemize}
\item brief mention of submodularity for structured sparsity regularization - most common application in machine learning
\end{itemize}
\fi


In Section~\ref{sec:Submodular} we introduce the notion of a submodular loss function in the context of empirical risk minimization.  The Structured Output SVM is one of the most popular objectives for empirical risk minimization of interdependent outputs, and we demonstrate its properties on non-modular loss functions in Section~\ref{sec:SOSVM}.  In Section~\ref{sec:Lovasz} we introduce the Lov\'{a}sz hinge as well as properties involving the convexity and computational complexity. We empirically demonstrate its performance first on a synthetic problem, then on image classification and labeling tasks on Pascal VOC dataset and the Microsoft COCO dataset 
%PASCAL VOC dataset\footnote{Additional experimental settings are demonstrated in the supplement due to space constraints.}
%{\color{red} and we empirically demonstrate its performance on a synthetic experiment motivated by early detection in a temporal sequence and a natural scene image dataset~\cite{zhou2007multi}}\todo{update this to actual applications.} 
in Section~\ref{sec:Results}.

\iffalse
\subsection{Related Work}


\fi


==> Lovasz.tex <==
\begin{figure*}[!htb] \centering
%%%%%%%%%%%%%%%%%%%%% plot of Lovasz hinge %%%%%%%%%%%%%%%%%
\subfigure{\label{fig:lsub+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01112}}}
\subfigure{\label{fig:lsub+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01112_}} }
\subfigure{\label{fig:lsub-1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular non-increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01104} }}
\subfigure{\label{fig:lsub-2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular non-increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01104_} }}\\
%%%%%%%%%%%%%%%% plot of margin&slack-rescaling %%%%%%%%%%%%%%
\subfigure{\label{fig:msub+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with submodular increasing $l$ ]
{\includegraphics[width=0.235\textwidth]{m_01112}}}
\subfigure{\label{fig:msub+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with submodular increasing $l$ ]
{\includegraphics[width=0.235\textwidth]{m_01112_}}}
\subfigure{\label{fig:msup+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with supermodular increasing $l$ ]
{\includegraphics[width=0.235\textwidth]{m_01128}}}
\subfigure{\label{fig:msup+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with supermodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{m_01128_}}}\\
\subfigure{\label{fig:ssub+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with submodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01112}}}
\subfigure{\label{fig:ssub+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with submodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01112_}}}
\subfigure{\label{fig:ssup+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with supermodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01128}}}
\subfigure{\label{fig:ssup+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with supermodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01128_}}}
%%%%%%%%%%%%%%%%%%% end of plot %%%%%%%%%%%%%%%%%%%%%%%
\caption{\label{fig:visualization} We introduce a novel convex surrogate for submodular losses, the Lov\'{a}sz hinge.  
We show here the Lov\'{a}sz hinge, margin and slack rescaling surfaces with different loss functions $l$ from different views; the $x$ and $y$ axes represent the value of $s_i^1$ and $s_i^2$  %respectively 
in Eq.~\eqref{eq:s_i_pi}; the $z$ axis represents the value of the convex surrogate; the solid red dots represent the values of $l$ at the vertices of the unit hypercube.  
%As the loss functions for slack and margin rescaling are increasing, 
The convex surrogate strategies yield extensions of the discrete loss.}% \ref{fig:msub-1} and \ref{fig:msub-2} for $l$ being submodular and non-increasing; \ref{fig:msup-1} and \ref{fig:msup-2} for $l$ being supermodular and non-increasing.}	
\end{figure*}
%%%%%%%%%%%%%%%%%%% end of plot margin-rescaling %%%%%%%%%%%%%%%%%%%%%%%
\section{Lov\'{a}sz Hinge}\label{sec:Lovasz}

We now construct a convex surrogate for submodular losses.  This surrogate is based on a fundamental result by Lov\'{a}sz relating submodular sets and piecewise linear convex functions. 
%
The Lov\'{a}sz extension allows the extension of a set-function defined on the vertices of the hypercube $\{0,1\}^p$ to the full hypercube $[0,1]^p$~\cite{lovasz1983submodular}: 
\begin{defin}\label{def:lovaszExt}
The Lov\'{a}sz extension $\hat{l}$ of a set function $l$, $\hat{l}:[0,1]^p\to\mathbb{R}$, is defined as follows: for  $s^{\pi}\in[0,1]^p$ with decreasing components $s^{\pi_1}\geq s^{\pi_2}\geq \cdots\geq s^{\pi_p}$ ordered by a permutation $\pi=(\pi_1,\pi_2,\cdots,\pi_p)$, $\hat{l}(s)$ is defined as:
\begin{equation}
\hat{l}(s)=\sum_{j=1}^{p} s^{\pi_j}\left(l\left(\{\pi_1,\cdots,\pi_j\}\right)-l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)
\end{equation}
\end{defin} 
It has been proven that a set-function $l$ is submodular iff its Lov\'{a}sz extension is convex~\cite{lovasz1983submodular}. Based on this definition, we propose our novel convex surrogate for submodular functions:
\begin{defin}\label{def:lovaszHing}
The Lov\'{a}sz hinge, $\mathbf{L}$, is defined as the unique operator such that, for $l$ submodular
\begin{align}
&\mathbf{L} \Delta(y,g(x)) :=\\
\nonumber
&\left(\max_{\pi}\sum_{j=1}^p s^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)\right)_+
\end{align}
where $(\cdot)_{+} = \max(\cdot,0)$, $\pi$ is a permutation,
\begin{equation}\label{eq:s_i_pi}
s^{\pi_j} = 1-g^{\pi_j}(x) y^{\pi_j},
\end{equation}
and $g^{\pi_j}(x)$ is the $\pi_j$th dimension of $g(x)$.
\end{defin}
%
\iffalse
\begin{defin}\label{def:lovaszHing}
The Lov\'{a}sz hinge %, $\mathbf{L} l$, 
regularized risk is defined as
\begin{align*}%\label{eq:marginrescal}
&\min_{w,\xi}  \frac{1}{2} \|w\|^2 + C \sum_{i=1}^{n} \xi_i,\qquad \text{s.t.}\ \forall i,\forall y\in \mathcal{Y},\\
&\xi_i \geq \max_{\pi} \sum_{k=1}^p s_i^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_k\}\right)- l\left(\{\pi_1,\cdots,\pi_{k-1}\}\right)\right)
\end{align*}
where $l$ is a submodular set function, $\pi=(\pi_1,\cdots,\pi_p)$ is a permutation of the index, and 
\begin{equation}
\label{eq:s_i_pi}
s_i^{\pi_j}=1-\langle w,x_i^{\pi_j}\rangle y_i^{\pi_j}
\end{equation}
\end{defin} 
\fi
%Denote $\gamma_{\pi_j}=l(\{\pi_1,\pi_2,\cdots,\pi_k\}) - l(\{\pi_1,\pi_2,\cdots,\pi_{k-1}\})$, then the 1-slack formulation constraint becomes $\xi \geq \sum_{i=1}^n \sum_{k=1}^p s^{\pi_k,i}\gamma_{\pi_j}$. 
%We note that if $l$ is submodular non-increasing, it implies $\xi\geq 0$; while $l$ is submodular increasing, there will be extra constraints/planes for the outside of the unit hypercube. We propose then to threshold negative components to zero iff $l$ is increasing. 
If $l$ is increasing, when $s_i^{\pi_j}$ becomes negative we may threshold the corresponding components to zero as in standard hinge loss.  %This will prevent the Lov\'{a}sz hinge from becoming negative outside the unit cube.  
%The Lov\'{a}sz hinge is itself an extension of the Lov\'{a}sz extension (defined over the $p$-dimensional unit cube) to $\mathbb{R}^p$.  
By thresholding negative $s_i^{\pi_j}$ to zero, we have that the Lov\'{a}sz hinge coincides exactly with slack rescaling in the special case of a modular loss, and coincides with an SVM in the case of Hamming loss. In the case that $l$ is non-increasing, the thresholding strategy no longer coincides with the Lov\'{a}sz extension over the unit cube, and will not yield an extension.  We therefore will not apply thresholding in the non-increasing case, but we still have that $\mathbf{L}\Delta \geq 0$ and is convex.\footnote{Source code is available for download at {\sourcecodeurl}.}
 % assuming that the minimum value attained by the loss function on a vertex of the unit cube is greater than or equal to zero.  This can always be enforced by adding a constant to the loss without changing its minimizer. %Lov\'{a}sz extension is defined of extension over unit cube, while our Lov\'{a}sz hinge is defined both on the interior and the exterior of the unit cube.
%In the situation that $l$ be modular, we claim that Lov\'{a}sz hinge is equivalent to slack rescaling.

As the computation of a cutting plane or loss gradient is precisely the same procedure as computing a value of the Lov\'{a}sz extension, we have the same computational complexity, which is $\mathcal{O}(p \log p)$ to sort the $p$ coefficients, followed by $\mathcal{O}(p)$ oracle accesses to the loss function~\cite{lovasz1983submodular}. This is precisely an application of the greedy algorithm to optimize a linear program over the submodular polytope~\cite{edmonds1971matroids}.  In our implementation, we have employed a one-slack cutting-plane optimization with $\ell_2$ regularization analogous to~\cite{Joachims/etal/09a}.  We observe empirical convergence of the primal-dual gap at a rate comparable to that of a structured output SVM (Fig.~\ref{fig:gap}).

\subsection{Visualization of convex surrogates}\label{sec:visual}

For visualization of the loss surfaces, in this section we consider a simple binary classification problem with two elements %($p=2$) 
with a non-modular loss function $l$:
\begin{displaymath}
\mathcal{X}:=\mathbb{R}^{d\times2}\qquad \mathcal{Y}:= \{-1,+1\}^2
\end{displaymath}
Then with different values for $l(\varnothing)$, $l(\{1\})$, $l(\{2\})$ and  $l(\{1,2\})$, we can have different modularity or monotonicity properties of the function $l$ which then defines $\Delta$. We illustrate the Lov\'{a}sz hinge, slack and margin rescaling for the following cases:
\begin{inparaenum}[(i)]
\item submodular increasing: $l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=1.2$,
\item submodular non-increasing: $l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=0.4$, and
\item supermodular increasing: $l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=2.8$.
%\item submodular non-increasing: $l(\{a_1\})=1,l(\{a_2\})=1,l(\{a_1,a_2\})=0.4$
%\item supermodular non-increasing: $l(\varnothing)=2.8,l(\{a_1\})=1,l(\{a_2\})=1,l(\{a_1,a_2\})=0$.
\end{inparaenum}

In Fig.~\ref{fig:visualization}, the $x$ axis represents the value of $s_i^1$, the $y$ axis represents the value of $s_i^2$ in Eq~\eqref{eq:s_i_pi}, and the $z$ axis is the convex loss function given by Equation~\eqref{eq:upbound_m}, Equation~\eqref{eq:upbound_s}, and Definition~\ref{def:lovaszHing}, respectively. We plot the values of $l$ as solid dots at the vertices of the hypercube. We observe that all the solid dots \emph{touch} the surfaces, which empirically validates that the surrogates are extensions of the discrete loss. Here we set $l$ as symmetric functions, while the extensions can be also validated for asymmetric increasing set functions. %We can observe that for margin rescaling (while having a proper positive scale factor $\gamma$), the dots coincide with the surfaces only for submodular increasing and supermodular increasing $l$; for the Lov\'{a}sz hinge, it is the case for submodular increasing as well. 

==> LovaszArXiv.tex <==
\begin{figure*}[!htb] \centering
%%%%%%%%%%%%%%%%%%%%% plot of Lovasz hinge %%%%%%%%%%%%%%%%%
\subfigure[Lov\'{a}sz hinge with submodular increasing $l$\label{fig:lsub+1}]
{\includegraphics[width=0.235\textwidth]{l_01112black.pdf}
\includegraphics[width=0.235\textwidth]{l_01112black_.pdf}}
\subfigure[Lov\'{a}sz hinge with submodular non-increasing $l$\label{fig:lsub-1}]
{\includegraphics[width=0.235\textwidth]{l_01104black.pdf}
\includegraphics[width=0.235\textwidth]{l_01104black_.pdf}}\\
%%%%%%%%%%%%%%%% plot of margin&slack-rescaling %%%%%%%%%%%%%%
\subfigure[Margin-rescaling with submodular increasing $l$\label{fig:msub+1}]
{\includegraphics[width=0.235\textwidth]{m_01112black.pdf}
\includegraphics[width=0.235\textwidth]{m_01112black_.pdf}}
\subfigure[Margin-rescaling with supermodular increasing $l$\label{fig:msup+1}]
{\includegraphics[width=0.235\textwidth]{m_01128black.pdf}
\includegraphics[width=0.235\textwidth]{m_01128black_.pdf}}\\
\subfigure[Slack-rescaling with submodular increasing $l$\label{fig:ssub+1}]
{\includegraphics[width=0.235\textwidth]{s_01112black.pdf}
\includegraphics[width=0.235\textwidth]{s_01112black_.pdf}}
\subfigure[Slack-rescaling with supermodular increasing $l$\label{fig:ssup+1}]
{\includegraphics[width=0.235\textwidth]{s_01128black.pdf}
\includegraphics[width=0.235\textwidth]{s_01128black_.pdf}}
%%%%%%%%%%%%%%%%%%% end of plot %%%%%%%%%%%%%%%%%%%%%%%
\caption{\label{fig:visualization} We introduce a novel convex surrogate for submodular losses, the Lov\'{a}sz hinge.  
We show here the Lov\'{a}sz hinge, margin and slack rescaling surfaces with different loss functions $l$ from different views; the $x$ and $y$ axes represent the value of $s_i^1$ and $s_i^2$ 
in Eq.~\eqref{eq:s_i_pi}; the $z$ axis represents the value of the convex surrogate; the solid red dots represent the values of $l$ at the vertices of the unit hypercube.  
The convex surrogate strategies yield extensions of the discrete loss.}
\end{figure*}
%%%%%%%%%%%%%%%%%%% end of plot margin-rescaling %%%%%%%%%%%%%%%%%%%%%%%
\section{Lov\'{a}sz Hinge}\label{sec:Lovasz}

\subsection{Lov\'{a}sz extension}\label{sec:lovaszextension}

In this section, we introduce a novel convex surrogate for submodular losses.  This surrogate is based on a fundamental result relating submodular sets and piecewise linear convex functions, called the Lov\'{a}sz extension~\cite{lovasz1983submodular}. It allows the extension of a set function defined on the vertices of the hypercube $\{0,1\}^p$ to the full hypercube $[0,1]^p$: 
\begin{defin}\label{def:lovaszExt}
The Lov\'{a}sz extension $\hat{l}$ of a set function $l$, $\hat{l}:[0,1]^p\to\mathbb{R}$, is defined as follows: for  $s^{\pi}\in[0,1]^p$ with decreasing components $s^{\pi_1}\geq s^{\pi_2}\geq \cdots\geq s^{\pi_p}$ ordered by a permutation $\pi=(\pi_1,\pi_2,\cdots,\pi_p)$, $\hat{l}(s)$ is defined as:
\begin{equation}
\hat{l}(s)=\sum_{j=1}^{p} s^{\pi_j}\left(l\left(\{\pi_1,\cdots,\pi_j\}\right)-l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)
\end{equation}
\end{defin} 

The Lov\'{a}sz extension connects submodular set functions and convex functions. Furthermore, we may substitute convex optimization of the Lov\'{a}sz extension for discrete optimization of a submodular set function:
% compute subgradient == compute a lovasz extension
% max pi == sorting s
\begin{pro}[Greedy algorithm~\cite{lovasz1983submodular,edmonds1971matroids}]\label{pro:lovaszExtensionGreedy}
For a submodular function $l$ such that $l(\emptyset)=0$,  $s^{\pi}\in\mathbb{R}^p$ with decreasing components $s^{\pi_1}\geq s^{\pi_2}\geq \cdots\geq s^{\pi_p}$ with a permutation $\pi$, and denote $\gamma_{\pi_j} = l\left(\{\pi_1,\cdots,\pi_j\}\right)-l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$, then $\gamma\in B(l)$ % in the base polyhedron in Definition 2.2 in Bach2013submodular
 and, 
 \begin{enumerate}[(i)]
  \item if $s\in \mathbb{R}^p_+$, $\gamma$ is a maximizer of $\max_{\gamma\in B(l)} s^\intercal\gamma$; $\max_{\gamma\in B(l)} s^\intercal\gamma = \hat{l}(s)$;
 \item $\gamma$ is a maximizer of $\max_{\gamma\in P(l)} s^\intercal\gamma$; $\max_{\gamma\in P(l)} s^\intercal\gamma = \hat{l}(s)$;
 \end{enumerate}
where $P(l)=\{s\in\mathbb{R}^p, \forall A\subseteq V, s(A)\leq l(A)\}$ is called the submodular polyhedron, and $B(l)=P(l)\cap\{s(V)=l(V)\}$ is called the base polyhedron.
%A maximizer of the Lov\'{a}sz extension can be obtained by sorting the components of $s$ as $s^{\pi_1}\geq s^{\pi_2}\geq \cdots\geq s^{\pi_p}$
\end{pro}
A proof with detailed analysis can be found in~\cite[Proposition 3.2 to 3.5]{bach2013submodular}.
That is to say, to find a maximum of $s^\intercal \gamma$, which is the same procedure as computing a subgradient of the Lov\'{a}sz extension, is precisely the following procedure:
\begin{enumerate}[(i)]
\item sort the $p$ components of $s$, which is in $\mathcal{O}(p \log p)$;
\item compute the value of $s^\intercal \gamma$ which needs $\mathcal{O}(p)$ oracle accesses to the set function. 
\end{enumerate} 

\begin{pro}[Convexity and submodularity~\cite{lovasz1983submodular}]\label{pro:lovaszExtensionConvex}
%It has been proven that a set-function $l$ is submodular iff its Lov\'{a}sz extension is convex~\cite{lovasz1983submodular}. 
A function l is submodular if and only if the Lov\'{a}sz extension $\hat{l}$ of l is convex.
\end{pro}
A proof of this proposition is given in~\cite[Proposition 3.6]{bach2013submodular}.
We then take the advantage of this proposition to define a novel convex surrogate for submodular loss functions.

\subsection{Lov\'{a}sz hinge}\label{sec:lovaszhinge}

We propose our novel convex surrogate for submodular functions increasing and non-increasing in Definition~\ref{def:lovaszHingIn} and Definition~\ref{def:lovaszHingNonIn}, respectively.\footnote{Source code is available for download at {\sourcecodeurl}.}
% increasing loss functions
\begin{defin}\label{def:lovaszHingIn}
For $l$ submodular and \emph{increasing}, the Lov\'{a}sz hinge $\mathbf{L}$ is defined as the unique operator such that, 
\begin{align}
\mathbf{L} \Delta(y,g(x)) := \label{eq:lovaszHingIn}
\max_{\pi}\sum_{j=1}^p \left(s^{\pi_j}\right)_+ \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)
\end{align}
where $(\cdot)_{+} = \max(\cdot,0)$, $\pi$ is a permutation,
\begin{equation}\label{eq:s_i_pi}
s^{\pi_j} = 1-g^{\pi_j}(x) y^{\pi_j},
\end{equation}
and $g^{\pi_j}(x)$ is the $\pi_j$th dimension of $g(x)$ (cf.\ Equation~\eqref{eq:g_func_x}).
\end{defin}

% non-increasing loss functions (may be interesting in some cases)
\begin{defin}\label{def:lovaszHingNonIn}
For $l$ submodular and \emph{non-increasing}, the Lov\'{a}sz hinge, $\mathbf{L}$, is defined as the unique operator such that 
\begin{align}
\mathbf{L} \Delta(y,g(x)) := \label{eq:lovaszHingNonIn}
\left(\max_{\pi}\sum_{j=1}^p s^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)\right)_+
\end{align}
with the same $\pi$, $s^{\pi_j}$, $g^{\pi_j}(x)$ and $(\cdot)_{+}$ defined as in Definition~\ref{def:lovaszHingIn}.
\end{defin}

Note that the Lov\'{a}sz hinge is itself an extension of the Lov\'{a}sz extension (defined over the $p$-dimensional unit cube) to $\mathbb{R}^p$.  
For $l$ being submodular increasing, we threshold each negative component of $s$ i.e.\ $s^{\pi_j} = 1-g^{\pi_j}(x) y^{\pi_j}$ to zero. As $l$ being increasing, the components $l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ will always be non-negative. Then $\mathbf{L} \Delta(y,g(x))$ in Defintion~\ref{def:lovaszHingIn} is always non-negative.  While in Definition~\ref{def:lovaszHingNonIn}, we don't apply the thresholding strategy on the components of $s$, but instead on the entire formulation. 

We show in the following propositions that these two definitions yield surrogates that are indeed convex and extensions of the corresponding loss functions.

\begin{pro}\label{pro:lovaszHingeNonIncreasing}
For a submodular non-negative loss function $l$, the Lov\'{a}sz hinge as in Definition~\ref{def:lovaszHingNonIn} is convex and yields an extension of $\Delta$
\end{pro}
\begin{proof}
We first demonstrate the ``convex'' part.
It is clear that taking a maximum over linear functions is convex. 
The thresholding to positive values similarly maintains convexity.
%Actually, as the Lov\'{a}sz hinge has the same manner as the Lov\'{a}sz extension inside the unitcube in $\mathbb{R}^p$ , it is should be always convex for submodular set function if there is no thresholding on the variable $s$, as in Definition~\ref{def:lovaszHingNonIn}.  

We then demonstrate the ``extension'' part. %it is precisely the same procedure as in the proof of Proposition~\ref{pro:lovaszHingeIncreasing};
From the definition of extension as in Equation~\eqref{eq:mapping2unitcube} as well as the notation concerning the vertices of the unit cube as in Equation~\eqref{eq:l_dot_gene}, for the values of $s$ on the vertices $\mathbf{I}$,  we have explicitly 
\begin{equation}\label{eq:sequals}
s^{j} = \left\{
\begin{array}{ll}
1,& \ \forall j\in\mathbf{I} \\
0,& \ \forall j\in V\setminus\mathbf{I}  
\end{array} \right.
\end{equation}
As a result, the permutation $\pi$ that sorts the components of $s$ decreasing on the vertices is actually 
\begin{displaymath}
\{\pi_1,\cdots,\pi_k, \pi_{k+1},\cdots,\pi_p\},\ k=|\mathbf{I}|.
\end{displaymath}
with $\{\pi_1,\cdots,\pi_k\}$ a permutation of $\{j|j\in\mathbf{I}\}$ and $\{\pi_{k+1},\cdots,\pi_p\}$ a permutation of $\{j|j\in V\setminus\mathbf{I}\}$.

We then reformulate the inside part of rhs of Equation~\eqref{eq:lovaszHingNonIn} as:
\begin{align}
&\sum_{j=1}^p s^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right) \nonumber\\
& = \sum_{j=1}^k 1\times \left( l\left(\{\pi_1,\cdots,\pi_k\}\right)- l\left(\{\pi_1,\cdots,\pi_{k-1}\}\right)\right) + 0 \nonumber\\
%& = \sum_{j=1}^{p-1} \left(s^{\pi_j}-s^{\pi_{j+1}}\right) l\left(\{\pi_1,\cdots,\pi_j\}\right) + s^{\pi_p} l(V). \label{eq:def6extension1} \\
& = l\left(\{\pi_1,\cdots,\pi_k\}\right) \nonumber\\
& = l(\mathbf{I})  \label{eq:def6extension2}
\end{align}
Then for non-negative $l$ the thresholding to positive is redundant. As a consequence we have  
\begin{equation}
\mathbf{L} \Delta(y,g(x)) = \left(l(\mathbf{I}) \right)_+ =  \Delta(y,g(x))
\end{equation} 
which validates that $\mathbf{L} \Delta(y,g(x))$ yields an extension of $\Delta(y,g(x))$.
\end{proof}

\begin{pro}\label{pro:lovaszHingeIncreasing}
For a submodular increasing loss function $l$ , the Lov\'{a}sz hinge as in Definition~\ref{def:lovaszHingIn} is convex and yields an extension of $\Delta$.
\end{pro}
\begin{proof}
We first demonstrate the ``convex'' part.
When $l$ is increasing, $\gamma^{\pi_j} = l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ will always be positive for all $\pi_j\in\{1,2,\cdots,p \}$. So it's obvious that $\gamma^{\pi_j}\times\max(0,s^{\pi_j})$ will always be convex with respect to $s^{\pi_j}\in\mathbb{R}$ for any given $\gamma^{\pi_j}\geq 0$. As the convex function set is closed under the operation of addition, the Lov\'{a}sz hinge is convex in $\mathbb{R}^p$.

We note that on the vertex $\mathbf{I}$, we have $s \in \{0,1\}^p$ as in Equation~\eqref{eq:sequals}, then the positive threshold on the components of $s^j$ can be removed. With a same procedure as in Equation~\eqref{eq:def6extension2}, $\mathbf{L} \Delta(y,g(x))$ yields an extension of $\Delta(y,g(x))$.

\end{proof}

\iffalse
\begin{pro}[Convexity]\label{pro:lovaszHingeIsConvex}
The Lov\'{a}sz hinge as in Definition~\ref{def:lovaszHingIn} is convex if and only if $l$ is increasing.
%For a submodular increasing loss function $l$ namely $\Delta$, the Lov\'{a}sz hinge is convex. 
%For a submodular non-increasing loss function $l$ namely $\Delta$, the Lov\'{a}sz hinge is \emph{not} convex if we threshold each negative component $s^{\pi_j}$ to zero. 
\end{pro}
\begin{proof}
We first demonstrate the ``if'' direction. 
If $l$ is increasing, $\gamma^{\pi_j} = l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ will always be positive for all $\pi_j\in\{1,2,\cdots,p \}$. So it's obvious that $\gamma^{\pi_j}\times\max(0,s^{\pi_j})$ will always be convex with respect to $s^{\pi_j}\in\mathbb{R}$ for any given $\gamma^{\pi_j}\geq 0$. Thus the Lov\'{a}sz hinge is convex in $\mathbb{R}^p$.

We then demonstrate the ``only if'' direction by contradiction. 
If $l$ is non-increasing, there exists at least one $\gamma^{\pi_j} = l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ that is strict negative. Then it's easy to verify that $\gamma^{\pi_j}\times\max(0,s^{\pi_j})$ is concave with respect to $s^{\pi_j}\in\mathbb{R}$ for this $\gamma^{\pi_j}< 0$. 

\end{proof}

\begin{pro}[Extension]\label{pro:lovaszHingeIsExtension}
For a submodular increasing (non-increasing) loss function $l$ namely $\Delta$, the Lov\'{a}sz hinge in Definition~\ref{def:lovaszHingIn} (Definition~\ref{def:lovaszHingNonIn}) is an extension of $\Delta$. 
% $\mathbf{L}\Delta$ is \emph{not} an extension of $\Delta$ if we threshold each negative component $s^{\pi_j}$ to zero. 
\end{pro}
\begin{proof}
We note that at the vertices of the unitcube in $\mathbb{R}^p$, $s$ has the component equal to $1$ at the dimension relating that specific vertex, and equal to $0$ otherwise. For example, at the vertex $\mathbf{I}=\{j\}$ (cf.\ Equation~\ref{eq:l_dot_gene}), we have $s^j = 1-g^j(x) y^j = 1$ (cf.\ Definition~\ref{def:extention}). We have then the sorted $s^\pi$ as $s^j=1\geq s^{j\neq 1}=0\geq \cdots$, with the $\pi$ has $j$ at the first place with $s^j=1$ and all $0$ otherwise. That's to say,
\begin{align}
\mathbf{L} \Delta(y,g(x)) 
&= s^j\left( l\left(\{j\}\right)- l\left(\emptyset \right)\right) \nonumber\\
&= 1\times l\left(\{j\}\right) \nonumber\\
&=\Delta(y,g(x))
\end{align}
which validates the definition of extension.
\end{proof}
\fi

Although Definition~\ref{def:lovaszHingNonIn} is convex and yields an extension for both increasing and non-increasing losses,  we rather apply Definition~\ref{def:lovaszHingIn} for increasing loss functions.
%If $l$ is submodular increasing, there will be extra constraints/planes for the outside of the unit hypercube, while if $l$ is submodular non-increasing, it implies $\xi\geq 0$. We propose then to threshold negative components to zero iff $l$ is increasing. 
This will ensure the Lov\'{a}sz hinge is an analogue to a standard hinge loss in the special case of a symmetric modular loss. 
We formally state this as the following proposition:
\begin{pro}
For a submodular increasing loss function $l$, the Lov\'{a}sz hinge as in Definition~\ref{def:lovaszHingIn} thresholding negative $s^{\pi_j}$ to zero, coincides with an SVM (i.e.\ additive hinge loss) in the case of Hamming loss. 
\end{pro}
\begin{proof}
The hinge loss for a set of $p$ training samples is defined to be
\begin{equation}
\ell_{\text{hinge}}(y,g(x)) := \sum_{i=1}^{p} \left(1-g(x^i) y^i )\right)_{+} .
\end{equation}
Following the previous notation, we will interpret $g(x^i) = g^i(x)$.  For a modular loss, the Lov\'{a}sz hinge in Equation~\eqref{eq:lovaszHingIn} simplifies to
\begin{eqnarray}
\mathbf{L}\Delta(y,g(x)) &=& \max_\pi \sum_{j=1}^p (s^{\pi_j})_+ l(\{\pi_j\})\\
&=& \sum_{j=1}^p \left( 1-g^j(x) y^j \right)_+ l(\{j\}) .
\end{eqnarray}
For the Hamming loss $l(\{j\}) = 1, \forall j$ and $\mathbf{L}\Delta(y,g(x)) = \ell_{\text{hinge}}(y,g(x))$.
\end{proof}


\begin{lem}\label{lem:LovaszConvexClosure}
The Lov\'{a}sz extension of a submodular function $l$ corresponds with the convex closure~\cite{bach2013submodular}.
\end{lem}

\begin{pro}\label{pro:LovaszHigherInsideCube}
The Lov\'{a}sz hinge has an equal or higher value than slack and margin rescaling inside the unit cube.
\end{pro}
\begin{proof}
By Lemma~\ref{lem:LovaszConvexClosure} it is clear that the Lov\'{a}sz hinge inside the unit cube is the maxim convex extension, and therefore slack and margin rescaling must have equal or lesser values.
\end{proof}
\begin{cor}
Slack and margin rescaling have additional inflection points inside the unit cube that are not present in the Lov\'{a}sz hinge.  This is a consequence of Proposition~\ref{pro:LovaszHigherInsideCube} and the fact that all three are piecewise linear extensions, and thus have identical values on the vertices of the unit cube. One can also visualize this in Figure~\ref{fig:visualization}.
\end{cor}

\iffalse
In the case that $l$ is non-increasing, the thresholding strategy no longer coincides with the Lov\'{a}sz extension over the unit cube, and will not yield an extension.  We therefore will not apply thresholding in the non-increasing case, but we still have that $\mathbf{L}\Delta \geq 0$ and is convex.
\begin{pro}
For a submodular non-increasing loss function $l$ namely $\Delta$, the Lov\'{a}sz hinge cannot yield extension if we still threshold each negative component $s^{\pi_j}$ to zero. 
\end{pro}
\fi

Another reason that we use a different threshold strategy on $s$ for increasing or non-increasing losses is that we cannot guarantee that the Lov\'{a}sz hinge is always convex if we threshold each negative component $s^{\pi_j}$ to zero for non-increasing losses. 

\begin{pro}\label{pro:lovaszHingeNonInIsConvex}
For a submodular non-increasing loss function $l$ , the Lov\'{a}sz hinge is \emph{not} convex if we threshold each negative component $s^{\pi_j}$ to zero as in Definition~\ref{def:lovaszHingIn}.
\end{pro}
\begin{proof}
If $l$ is non-increasing, there exists at least one $\pi$ and $j$ such that $\delta_{\pi}^{j} := l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ is strictly negative.
The partial derivative of $\mathbf{L}\Delta(y,g(x))$ w.r.t.\ $s^{\pi_j}$ is
\begin{equation}
\frac{\partial \mathbf{L}\Delta(y,g(x))}{\partial s^{\pi_j}} = \begin{cases} 0 & \text{if } s^{\pi_j} <0 \\
\delta_{\pi}^{j} & \text{if } s^{\pi_j} >0 .
\end{cases}
\end{equation}
As $\delta_{\pi}^{j} < 0$ by assumption, we have that the partial derivative at $s^{\pi_j} <0$ is larger than the partial derivative at $s^{\pi_j} >0$, and the loss surface cannot therefore be convex.
\end{proof}

Figure~\ref{fig:lsub-3} and Figure~\ref{fig:lsub-4} show an example of the loss surface when $l$ is non-increasing. We can see that at the non-increasing element leads to a negative subgradient at one side of a vertex, while on its other side the subgradient is zero due to the fact that we still apply the thresholding strategy. Thus it leads to a non-convex surface. 


% assuming that the minimum value attained by the loss function on a vertex of the unit cube is greater than or equal to zero.  This can always be enforced by adding a constant to the loss without changing its minimizer. %Lov\'{a}sz extension is defined of extension over unit cube, while our Lov\'{a}sz hinge is defined both on the interior and the exterior of the unit cube.
%In the situation that $l$ be modular, we claim that Lov\'{a}sz hinge is equivalent to slack rescaling.

\subsection{Complexity of subgradient computation}
%In practice, regarding using the cutting plane algorithm, the 1-slack formulation constraint becomes \begin{equation}
%\xi_i \geq \max_{\pi} \sum_{j=1}^p s_i^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right).
%\end{equation} 
% max_pi == sort pi

We explicitly present the cutting plane algorithm for solving the max-margin problem as in Equation~\eqref{eq:maxmargin} in Algorithm~\ref{alg:cuttingplanLovasHinge}. The novelties are: (i) in Line~\ref{algline:setLovaszHinge} we calculate the upper bound on the empirical loss by the Lov\'{a}sz hinge; (ii) in Line~\ref{algline:LovaszHingeSubgradient} we calculate the loss gradient by the computation relating to the permutation $\pi$ instead of to all possible outputs $\tilde{y}$.
\begin{algorithm}[!t]
\caption{Cutting plane algorithm for solving the problem in Equation~\eqref{eq:maxmargin}, with Definition~\ref{def:lovaszHingNonIn} -- the Lov\'{a}sz hinge.}\label{alg:cuttingplanLovasHinge}
\begin{algorithmic}[1]
\STATE {Input: $(x_1,y_1),\cdots,(x_n,y_n),C,\epsilon$}
\STATE $S^i = \emptyset, \forall i = 1,\cdots,n$
\REPEAT 
\STATE for $i=1,\cdots,n$ do
\STATE \label{algline:setLovaszHinge} $H(y_i) = \sum_{j=1}^p s_i^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right) $, where $s^{\pi_j} = 1-g^{\pi_j}(x_i) y_i^{\pi_j}$
\STATE \label{algline:LovaszHingeSubgradient} $\hat{y} = \arg\max_{\pi} H(y_i)$ \% find the most violated constraint by sorting the p elements
\STATE $\xi^i = \max\{0,H(y_i)\}$
\IF {$H(\hat{y})>\xi^i+\epsilon$ }
\STATE $S^i:=S^{i}\cup \{y_i\}$
\STATE $w\leftarrow$ optimize Equation~\eqref{eq:maxmargin} with constraints defined by $\cup_i S^i$
\ENDIF
\UNTIL{no $S^i$ has changed during iteration}
\RETURN $(w,\xi)$
\end{algorithmic}  
\end{algorithm}

As the computation of a cutting plane or loss gradient is precisely the same procedure as computing a value of the Lov\'{a}sz extension, we have the same computational complexity, which is $\mathcal{O}(p \log p)$ to sort the $p$ coefficients, followed by $\mathcal{O}(p)$ oracle accesses to the loss function~\cite{lovasz1983submodular}. %This is precisely an application of the greedy algorithm to optimize a linear program over the submodular polytope~\cite{edmonds1971matroids}.  
This is precisely an application of the greedy algorithm to optimize a linear program over the submodular polytope as shown in Proposition~\ref{pro:lovaszExtensionGreedy}.
In our implementation, we have employed a one-slack cutting-plane optimization with $\ell_2$ regularization analogous to~\cite{Joachims/etal/09a}.  We observe empirical convergence of the primal-dual gap at a rate comparable to that of a structured output SVM (Fig.~\ref{fig:gap}).

\begin{figure}[!t] \centering
%%%%%%%%%%%%%%%%%%%%% plot of Lovasz hinge %%%%%%%%%%%%%%%%%
\subfigure{\label{fig:lsub-3}% Lov\'{a}sz hinge with submodular non-increasing $l$]
\includegraphics[width=0.35\textwidth]{l_01104thresholdingblack.pdf}}
\subfigure{\label{fig:lsub-4}% Lov\'{a}sz hinge with submodular non-increasing $l$]
\includegraphics[width=0.35\textwidth]{l_01104thresholdingblack_.pdf}}
%%%%%%%%%%%%%%%%%%% end of plot %%%%%%%%%%%%%%%%%%%%%%%
\caption{\label{fig:increasingLovaszHingewithNonIncreasingl} 
 Lov\'{a}sz hinge with submodular non-increasing $l$ while thresholding negative components of $s$ is still applied (cf.\ the caption of Figure~\ref{fig:visualization} for the axes notation). Although the red dots touch the surface, the surface is no longer convex due to the thresholding strategy.}% \ref{fig:msub-1} and \ref{fig:msub-2} for $l$ being submodular and non-increasing; \ref{fig:msup-1} and \ref{fig:msup-2} for $l$ being supermodular and non-increasing.}	
\end{figure}

\subsection{Visualization of convex surrogates}\label{sec:visual}

For visualization of the loss surfaces, in this section we consider a simple binary classification problem with two elements %($p=2$) 
with non-modular loss functions :
\begin{displaymath}
\mathcal{X}:=\mathbb{R}^{d\times2}\qquad \mathcal{Y}:= \{-1,+1\}^2
\end{displaymath}
Then with different values for $l(\varnothing)$, $l(\{1\})$, $l(\{2\})$ and  $l(\{1,2\})$, we can have different modularity or monotonicity properties of the function $l$ which then defines $\Delta$. We illustrate the Lov\'{a}sz hinge, slack and margin rescaling for the following cases:
%\begin{inparaenum}[(i)]
\begin{enumerate}[(i)]
\item submodular increasing: \\$l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=1.2$,
\item submodular non-increasing: \\$l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=0.4$, and
\item supermodular increasing: \\$l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=2.8$.
%\item submodular non-increasing: $l(\{a_1\})=1,l(\{a_2\})=1,l(\{a_1,a_2\})=0.4$
%\item supermodular non-increasing: $l(\varnothing)=2.8,l(\{a_1\})=1,l(\{a_2\})=1,l(\{a_1,a_2\})=0$.
\end{enumerate}
%\end{inparaenum}

In Fig.~\ref{fig:visualization}, the $x$ axis represents the value of $s^1$, the $y$ axis represents the value of $s^2$ in Eq~\eqref{eq:s_i_pi}, and the $z$ axis is the convex loss function given by Equation~\eqref{eq:upbound_m}, Equation~\eqref{eq:upbound_s}, and~\cref{def:lovaszHingIn,def:lovaszHingNonIn} for different loss functions. We plot the values of $l$ as solid dots at the vertices of the hypercube. 

We observe first that all surfaces are convex. For the Lov\'{a}sz hinge with submodular increasing function in Figure~\ref{fig:lsub+1} and Figure~\ref{fig:lsub+2}, the thresholding strategy adds two hyperplanes on the left and on the right, while convexity is maintained.
We observe then that all the solid dots corresponding to the discrete loss fuction values \emph{touch} the surfaces, which empirically validates that the surrogates are extensions of the discrete loss. Here we set $l$ as symmetric functions, while the extensions can be also validated for asymmetric increasing set functions. 

We additionally plot the Lov\'{a}sz hinge with the non-increasing function while the thresholding strategy on $s$ is still applied, in Figure~\ref{fig:increasingLovaszHingewithNonIncreasingl}. Compared to Figure~\ref{fig:lsub-1}, convexity is lost due to the thresholding strategy on negative components of $s$.
%that for margin rescaling (while having a proper positive scale factor $\gamma$), the dots coincide with the surfaces only for submodular increasing and supermodular increasing $l$; for the Lov\'{a}sz hinge, it is the case for submodular increasing as well. 


==> LovaszPAMI_old.tex <==
\begin{figure*}[!htb] \centering
%%%%%%%%%%%%%%%%%%%%% plot of Lovasz hinge %%%%%%%%%%%%%%%%%
\subfigure{\label{fig:lsub+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01112}}}
\subfigure{\label{fig:lsub+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01112_}} }
\subfigure{\label{fig:lsub-1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular non-increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01104} }}
\subfigure{\label{fig:lsub-2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Lov\'{a}sz hinge with submodular non-increasing $l$]
{\includegraphics[width=0.23\textwidth]{l_01104_} }}\\
%%%%%%%%%%%%%%%% plot of margin&slack-rescaling %%%%%%%%%%%%%%
\subfigure{\label{fig:msub+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with submodular increasing $l$ ]
{\includegraphics[width=0.235\textwidth]{m_01112}}}
\subfigure{\label{fig:msub+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with submodular increasing $l$ ]
{\includegraphics[width=0.235\textwidth]{m_01112_}}}
\subfigure{\label{fig:msup+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with supermodular increasing $l$ ]
{\includegraphics[width=0.235\textwidth]{m_01128}}}
\subfigure{\label{fig:msup+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Margin-rescaling with supermodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{m_01128_}}}\\
\subfigure{\label{fig:ssub+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with submodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01112}}}
\subfigure{\label{fig:ssub+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with submodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01112_}}}
\subfigure{\label{fig:ssup+1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with supermodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01128}}}
\subfigure{\label{fig:ssup+2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ Slack-rescaling with supermodular increasing $l$]
{\includegraphics[width=0.235\textwidth]{s_01128_}}}
%%%%%%%%%%%%%%%%%%% end of plot %%%%%%%%%%%%%%%%%%%%%%%
\caption{\label{fig:visualization} We introduce a novel convex surrogate for submodular losses, the Lov\'{a}sz hinge.  
We show here the Lov\'{a}sz hinge, margin and slack rescaling surfaces with different loss functions $l$ from different views; the $x$ and $y$ axes represent the value of $s_i^1$ and $s_i^2$  %respectively 
in Eq.~\eqref{eq:s_i_pi}; the $z$ axis represents the value of the convex surrogate; the solid red dots represent the values of $l$ at the vertices of the unit hypercube.  
%As the loss functions for slack and margin rescaling are increasing, 
The convex surrogate strategies yield extensions of the discrete loss.}% \ref{fig:msub-1} and \ref{fig:msub-2} for $l$ being submodular and non-increasing; \ref{fig:msup-1} and \ref{fig:msup-2} for $l$ being supermodular and non-increasing.}	
\end{figure*}
%%%%%%%%%%%%%%%%%%% end of plot margin-rescaling %%%%%%%%%%%%%%%%%%%%%%%
\section{Lov\'{a}sz Hinge}\label{sec:Lovasz}

\subsection{Lov\'{a}sz extension}\label{sec:lovaszextension}

We now construct a novel convex surrogate for submodular losses.  This surrogate is based on a fundamental result relating submodular sets and piecewise linear convex functions, called the Lov\'{a}sz extension~\cite{lovasz1983submodular}. It allows the extension of a set function defined on the vertices of the hypercube $\{0,1\}^p$ to the full hypercube $[0,1]^p$: 
\begin{defin}\label{def:lovaszExt}
The Lov\'{a}sz extension $\hat{l}$ of a set function $l$, $\hat{l}:[0,1]^p\to\mathbb{R}$, is defined as follows: for  $s^{\pi}\in[0,1]^p$ with decreasing components $s^{\pi_1}\geq s^{\pi_2}\geq \cdots\geq s^{\pi_p}$ ordered by a permutation $\pi=(\pi_1,\pi_2,\cdots,\pi_p)$, $\hat{l}(s)$ is defined as:
\begin{equation}
\hat{l}(s)=\sum_{j=1}^{p} s^{\pi_j}\left(l\left(\{\pi_1,\cdots,\pi_j\}\right)-l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)
\end{equation}
\end{defin} 

The Lov\'{a}sz extension sets up the links between submodular set functions and convex functions, and benefits us with the convenience to use the convex analysis. Especially fundamental results are follows:
% compute subgradient == compute a lovasz extension
% max pi == sorting s
\begin{pro}[Greedy algorithm~\cite{lovasz1983submodular,edmonds1971matroids}]\label{pro:lovaszExtensionGreedy}
For a submodular function $l$ such that $l(\emptyset)=0$,  $s^{\pi}\in\mathbb{R}^p$ with decreasing components $s^{\pi_1}\geq s^{\pi_2}\geq \cdots\geq s^{\pi_p}$ with a permutation $\pi$, and denote $\gamma_{\pi_j} = l\left(\{\pi_1,\cdots,\pi_j\}\right)-l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$, then $\gamma\in B(l)$ % in the base polyhedron in Definition 2.2 in Bach2013submodular
 and, 
 \begin{enumerate}[(i)]
  \item if $s\in \mathbb{R}^p_+$, $\gamma$ is a maximizer of $\max_{\gamma\in B(l)} s^\intercal\gamma$; $\max_{\gamma\in B(l)} s^\intercal\gamma = \hat{l}(s)$;
 \item $\gamma$ is a maximizer of $\max_{\gamma\in P(l)} s^\intercal\gamma$; $\max_{\gamma\in P(l)} s^\intercal\gamma = \hat{l}(s)$;
 \end{enumerate}
where $P(l)=\{s\in\mathbb{R}^p, \forall A\subseteq V, s(A)\leq l(A)\}$ called the submodular polyhedron, and $B(l)=P(l)\cap\{s(V)=l(V)\}$ called the base polyhedron.
%A maximizer of the Lov\'{a}sz extension can be obtained by sorting the components of $s$ as $s^{\pi_1}\geq s^{\pi_2}\geq \cdots\geq s^{\pi_p}$
\end{pro}
A proof with detailed analysis can be found in~\cite[Proposition 3.2 to 3.5]{bach2013submodular}.
That's to say, to find a maximal of $s^\intercal \gamma$, which is the same as computing a subgradient, is precisely the procedure as follows:
\begin{enumerate}[(i)]
\item sort the $p$ components of $s$, which is in $\mathcal{O}(p \log p)$;
\item compute the value of $s^\intercal \gamma$ which needs $\mathcal{O}(p)$ oracle. 
\end{enumerate} 

\begin{pro}[Convexity and submodularity~\cite{lovasz1983submodular}]\label{pro:lovaszExtensionConvex}
%It has been proven that a set-function $l$ is submodular iff its Lov\'{a}sz extension is convex~\cite{lovasz1983submodular}. 
A function l is submodular if and only if the Lov\'{a}sz extension $\hat{l}$ of l is convex.
\end{pro}
A proof of this proposition is given in~\cite[Proposition 3.6]{bach2013submodular}.
We then take the advantage of this proposition to define a novel convex surrogate for submodular loss function.

\subsection{Lov\'{a}sz hinge}\label{sec:lovaszhinge}

We propose our novel convex surrogate for submodular functions increasing and non-increasing in Definition~\ref{def:lovaszHingIn} and Definition~\ref{def:lovaszHingNonIn}, respectively.
% increasing loss functions
\begin{defin}\label{def:lovaszHingIn}
The Lov\'{a}sz hinge, $\mathbf{L}$, is defined as the unique operator such that, for $l$ submodular and \emph{increasing}
\begin{align}
&\mathbf{L} \Delta(y,g(x)) :=\\
\nonumber
&\max_{\pi}\sum_{j=1}^p \left(s^{\pi_j}\right)_+ \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)
\end{align}
where $(\cdot)_{+} = \max(\cdot,0)$, $\pi$ is a permutation,
\begin{equation}\label{eq:s_i_pi}
s^{\pi_j} = 1-g^{\pi_j}(x) y^{\pi_j},
\end{equation}
and $g^{\pi_j}(x)$ is the $\pi_j$th dimension of $g(x)$.
\end{defin}

% non-increasing loss functions (may be interesting in some cases)
\begin{defin}\label{def:lovaszHingNonIn}
For $l$ submodular and \emph{non-increasing}, the Lov\'{a}sz hinge, $\mathbf{L}$, is defined as the unique operator such that 
\begin{align}
&\mathbf{L} \Delta(y,g(x)) :=\\
\nonumber
&\left(\max_{\pi}\sum_{j=1}^p s^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right)\right)_+
\end{align}
with the same $\pi$, $s^{\pi_j}$ and $g^{\pi_j}(x)$ defined as in Definition~\ref{def:lovaszHingIn}.
\end{defin}

Note that for $l$ being submodular increasing, we threshold each negative component of $s$ i.e.\ $s^{\pi_j} = 1-g^{\pi_j}(x) y^{\pi_j}$ to zero, then compute the Lov\'{a}sz hinge. As $l$ being increasing, the components $l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ will always be non-negative. Then $\mathbf{L} \Delta(y,g(x))$ is always non-negative. 

We explain the positive threshold as follows:
if $l$ is submodular increasing, there will be extra constraints/planes for the outside of the unit hypercube, while if $l$ is submodular non-increasing, it implies $\xi\geq 0$. We propose then to threshold negative components to zero iff $l$ is increasing. 
This will prevent the Lov\'{a}sz hinge from becoming negative outside the unit cube, which is an analogue to a standard hinge loss.
By thresholding negative $s_i^{\pi_j}$ to zero, we have that the Lov\'{a}sz hinge coincides exactly with slack rescaling in the special case of a modular loss, and coincides with an SVM in the case of Hamming loss. 
Note that the Lov\'{a}sz hinge is itself an extension of the Lov\'{a}sz extension (defined over the $p$-dimensional unit cube) to $\mathbb{R}^p$.  

In the case that $l$ is non-increasing, the thresholding strategy no longer coincides with the Lov\'{a}sz extension over the unit cube, and will not yield an extension.  We therefore will not apply thresholding in the non-increasing case, but we still have that $\mathbf{L}\Delta \geq 0$ and is convex.\footnote{Source code is available for download at {\sourcecodeurl}.}

\begin{pro}\label{pro:lovaszHingeIsExtension}
For a submodular increasing (non-increasing) loss function $l$ namely $\Delta$, the Lov\'{a}sz hinge in Definition~\ref{def:lovaszHingIn} (Definition~\ref{def:lovaszHingNonIn}) is an extension of $\Delta$. % $\mathbf{L}\Delta$ is \emph{not} an extension of $\Delta$ if we threshold each negative component $s^{\pi_j}$ to zero. 
\end{pro}
\begin{proof}
We note that at the vertices of the unitcube in $\mathcal{R}^p$, $s$ has the component equal to $1$ at the dimension relating that specific vertex, and equal to $0$ otherwise. For example, at the vertex $\mathbf{I}=\{j\}$ (cf.\ Equation~\ref{eq:l_dot_gene}), we have $s^j = 1-g^j(x) y^j = 1$ (cf.\ Definition~\ref{def:extention}). We have then the sorted $s^\pi$ as $s^j=1\geq s^{j\neq}=0\geq \cdots$, with the $\pi$ has $j$ at the first place with $s^j=1$ and all $0$ otherwise. That's to say,
\begin{align}
\mathbf{L} \Delta(y,g(x)) 
&= s^j\left( l\left(\{j\}\right)- l\left(\emptyset \right)\right) \nonumber\\
&= 1\times l\left(\{j\}\right) \nonumber\\
&=\Delta(y,g(x))
\end{align}
which validates the definition of extension.
\end{proof}

As the Lov\'{a}sz hinge has the same manner as the Lov\'{a}sz extension inside the unitcube in $\mathbb{R}^p$ , it is should be always convex for submodular set function if there is no thresholding on the variable $s$. We demonstrate that with the correct thresholding as in~\cref{def:lovaszHingIn,def:lovaszHingNonIn}, the Lov\'{a}sz hinge is convex.

\begin{pro}\label{pro:lovaszHingeInIsConvex}
For a submodular increasing loss function $l$ namely $\Delta$, the Lov\'{a}sz hinge is convex. 
\end{pro}
\begin{proof}
When $l$ is increasing, $\gamma^{\pi_j} = l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ will always be positive for all $\pi_j\in\{1,2,\cdots,p \}$. So it's obvious that $\gamma^{\pi_j}\times\max(0,s^{\pi_j})$ will always be convex with respect to $s^{\pi_j}\in\mathbb{R}$ for any given $\gamma^{\pi_j}\geq 0$. Thus the Lov\'{a}sz hinge is convex in $\mathbb{R}^p$.
\end{proof}

\begin{pro}\label{pro:lovaszHingeNonInIsConvex}
For a submodular non-increasing loss function $l$ namely $\Delta$, the Lov\'{a}sz hinge is \emph{not} convex if we threshold each negative component $s^{\pi_j}$ to zero. 
\end{pro}
\begin{proof}
When $l$ is non-increasing, there exists at least one $\gamma^{\pi_j} = l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)$ that is strict negative. Then it's easy to verify that $\gamma^{\pi_j}\times\max(0,s^{\pi_j})$ is concave with respect to $s^{\pi_j}\in\mathbb{R}$ for this $\gamma^{\pi_j}< 0$. Thus the Lov\'{a}sz hinge is not convex in $\mathbb{R}^p$.
\end{proof}
 % assuming that the minimum value attained by the loss function on a vertex of the unit cube is greater than or equal to zero.  This can always be enforced by adding a constant to the loss without changing its minimizer. %Lov\'{a}sz extension is defined of extension over unit cube, while our Lov\'{a}sz hinge is defined both on the interior and the exterior of the unit cube.
%In the situation that $l$ be modular, we claim that Lov\'{a}sz hinge is equivalent to slack rescaling.

\subsection{Complexity of subgradient computation}
%In practice, regarding using the cutting plane algorithm, the 1-slack formulation constraint becomes \begin{equation}
%\xi_i \geq \max_{\pi} \sum_{j=1}^p s_i^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right).
%\end{equation} 
% max_pi == sort pi

We explicitly present the cutting plane algorithm for solving the max-margin problem as in Equation~\eqref{eq:maxmargin} in Algorithm~\ref{alg:cuttingplanLovasHinge}. The novelties are: (i) in Line~\ref{algline:setLovaszHinge} we calculate the upper bound on the empirical loss by the convex operator Lov\'{a}sz hinge; (ii) in Line~\ref{algline:LovaszHingeSubgradient} we calculate the loss gradient by the computation relating to the permutation $\pi$ instead of to all possible output $\tilde{y}$.
\begin{algorithm}[!t]
\caption{Cutting plane algorithm for solving the problem in Equation~\eqref{eq:maxmargin}, with~\cref{def:lovaszHingIn,def:lovaszHingNonIn}  (i.e.\ with Lovasz hinge) }\label{alg:cuttingplanLovasHinge}
\begin{algorithmic}[1]
\STATE {Input: $(x_1,y_1),\cdots,(x_n,y_n),C,\epsilon$}
\STATE $S^i = \emptyset, \forall i = 1,\cdots,n$
\REPEAT 
\STATE for $i=1,\cdots,n$ do
\STATE \label{algline:setLovaszHinge} $H(y_i) = \sum_{j=1}^p s_i^{\pi_j} \left( l\left(\{\pi_1,\cdots,\pi_j\}\right)- l\left(\{\pi_1,\cdots,\pi_{j-1}\}\right)\right) $, where $s^{\pi_j} = 1-g^{\pi_j}(x_i) y_i^{\pi_j}$
\STATE \label{algline:LovaszHingeSubgradient} $\hat{y} = \arg\max_{\pi} H(y_i)$ \% find the most violate constraint by sorting the p elements
\STATE $\xi^i = \max\{0,H(y_i)\}$
\IF {$H(y)>\xi^i+\epsilon$ }
\STATE $S^i:=S^i\cup \{y_i\}$
\STATE $w\leftarrow$ optimize Equation~\eqref{eq:maxmargin} with constraints defined by $\cup_i S^i$
\ENDIF
\UNTIL{no $S^i$ has changed during iteration}
\RETURN $(w,\xi)$
\end{algorithmic}  
\end{algorithm}

As the computation of a cutting plane or loss gradient is precisely the same procedure as computing a value of the Lov\'{a}sz extension, we have the same computational complexity, which is $\mathcal{O}(p \log p)$ to sort the $p$ coefficients, followed by $\mathcal{O}(p)$ oracle accesses to the loss function~\cite{lovasz1983submodular}. %This is precisely an application of the greedy algorithm to optimize a linear program over the submodular polytope~\cite{edmonds1971matroids}.  
This is precisely an application of the greedy algorithm to optimize a linear program over the submodular polytope as shown in Proposition~\ref{pro:lovaszExtensionGreedy}.
In our implementation, we have employed a one-slack cutting-plane optimization with $\ell_2$ regularization analogous to~\cite{Joachims/etal/09a}.  We observe empirical convergence of the primal-dual gap at a rate comparable to that of a structured output SVM (Fig.~\ref{fig:gap}).

\subsection{Visualization of convex surrogates}\label{sec:visual}

For visualization of the loss surfaces, in this section we consider a simple binary classification problem with two elements %($p=2$) 
with non-modular loss functions :
\begin{displaymath}
\mathcal{X}:=\mathbb{R}^{d\times2}\qquad \mathcal{Y}:= \{-1,+1\}^2
\end{displaymath}
Then with different values for $l(\varnothing)$, $l(\{1\})$, $l(\{2\})$ and  $l(\{1,2\})$, we can have different modularity or monotonicity properties of the function $l$ which then defines $\Delta$. We illustrate the Lov\'{a}sz hinge, slack and margin rescaling for the following cases:
%\begin{inparaenum}[(i)]
\begin{enumerate}[(i)]
\item submodular increasing: \\$l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=1.2$,
\item submodular non-increasing: \\$l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=0.4$, and
\item supermodular increasing: \\$l(\varnothing)=0,\ l(\{1\})=l(\{2\})=1,\ l(\{1,2\})=2.8$.
%\item submodular non-increasing: $l(\{a_1\})=1,l(\{a_2\})=1,l(\{a_1,a_2\})=0.4$
%\item supermodular non-increasing: $l(\varnothing)=2.8,l(\{a_1\})=1,l(\{a_2\})=1,l(\{a_1,a_2\})=0$.
\end{enumerate}
%\end{inparaenum}

In Fig.~\ref{fig:visualization}, the $x$ axis represents the value of $s_i^1$, the $y$ axis represents the value of $s_i^2$ in Eq~\eqref{eq:s_i_pi}, and the $z$ axis is the convex loss function given by Equation~\eqref{eq:upbound_m}, Equation~\eqref{eq:upbound_s}, and~\cref{def:lovaszHingIn,def:lovaszHingNonIn}, respectively. We plot the values of $l$ as solid dots at the vertices of the hypercube. 

We observe first that all surfaces are convex. Especially the Lov\'{a}sz hinge with submodular increasing function in Figure~\ref{fig:lsub+1} and Figure~\ref{fig:lsub+2}, the thresholding strategy are adding two hyperplanes on the left and on the right, while the convexity is maintained.
We observe then that all the solid dots \emph{touch} the surfaces, which empirically validates that the surrogates are extensions of the discrete loss. Here we set $l$ as symmetric functions, while the extensions can be also validated for asymmetric increasing set functions. 

We additionally plot the Lov\'{a}sz hinge with the non-increasing function while the thresholding strategy is still applied, in Figure~\ref{fig:increasingLovaszHingewithNonIncreasingl}. Compare to Figure~\ref{fig:lsub-1} and Figure~\ref{fig:lsub-2}, the convexity is lost due to the thresholding strategy on negative components of $s$.
%that for margin rescaling (while having a proper positive scale factor $\gamma$), the dots coincide with the surfaces only for submodular increasing and supermodular increasing $l$; for the Lov\'{a}sz hinge, it is the case for submodular increasing as well. 

\begin{figure}[!t] \centering
%%%%%%%%%%%%%%%%%%%%% plot of Lovasz hinge %%%%%%%%%%%%%%%%%
\subfigure{\label{fig:lsub-3}% Lov\'{a}sz hinge with submodular non-increasing $l$]
\includegraphics[width=0.235\textwidth]{l_01104-crop}}
\subfigure{\label{fig:lsub-4}% Lov\'{a}sz hinge with submodular non-increasing $l$]
\includegraphics[width=0.235\textwidth]{l_01104_-crop}}
%%%%%%%%%%%%%%%%%%% end of plot %%%%%%%%%%%%%%%%%%%%%%%
\caption{\label{fig:increasingLovaszHingewithNonIncreasingl} 
 Lov\'{a}sz hinge with submodular non-increasing $l$ while thresholding negative components of $s$ is still applied (cf.\ the caption of Figure~\ref{fig:visualization} for the axes notation). Although the red dots touch the surface, the surface loss the convexity due to the thresholding strategy.}% \ref{fig:msub-1} and \ref{fig:msub-2} for $l$ being submodular and non-increasing; \ref{fig:msup-1} and \ref{fig:msup-2} for $l$ being supermodular and non-increasing.}	
\end{figure}

==> Results.tex <==
\section{Experimental Results}\label{sec:Results}
%\subsection{PASCAL VOC}
In this section, we consider a task in which multiple labels need to be predicted simultaneously and for which a submodular loss over labels is to be minimized.\footnote{Additional prediction tasks are demonstrated in the supplementary material due to space constraints.} Fig.~\ref{fig:voc} shows example images from the Pascal VOC dataset~\cite{pascal-voc-2007}, which include \textit{people}, \textit{tables} or \textit{chairs}. 
%Fig.\ref{fig:table} and Fig.\ref{fig:chair} contain all of these three categories/labels while Fig.\ref{fig:chaironly} contains only dining tables and chairs. 
If a subsequent prediction task focuses on detecting ``\textit{people sitting around a table}'', the initial multilabel prediction should emphasize that all labels must be correct \emph{within a given image}. This contrasts with a traditional multi-label prediction task in which a loss function decomposes over the individual predictions. The misprediction of a single label, e.g.\ \textit{person}, will preclude the chance to predict correctly the combination of all three labels. %The fact that the augmentation of mistakes doesn't make the prediction action equally worse. 
This corresponds exactly to the property of diminishing returns of a submodular function. 
 
While using classic modular losses such as 0-1 loss, the classifier is trained to minimize the sum of incorrect predictions, so the complex interaction between label mispredictions is not considered. In this work, we use a new submodular loss function and apply the Lov\'{a}sz hinge to enable efficient convex risk minimization.
\begin{figure}[t]  \centering
\subfigure{\label{fig:table}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.65in]{diningtable_04}}}
\subfigure{\label{fig:chair}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.65in]{chair_03}}}
\subfigure{\label{fig:chaironly}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.65in]{chair_01}}}
\caption{\label{fig:voc}Examples from the PASCAL VOC dataset. Fig.\ref{fig:table} and Fig.\ref{fig:chair} contain three categories: \textit{people}, \textit{table} and \textit{chair}. Fig.\ref{fig:chaironly} contains \textit{table} and \textit{chair}.}
\end{figure}

\paragraph{PASCAL VOC dataset} We use the PASCAL VOC~\cite{pascal-voc-2007} dataset for this prediction task. This challenging dataset contains around 10,000 images of 20 classes including animals, handmade and natural objects. In our work, we choose the most common combination of three categories: \textit{person}, \textit{chairs} and \textit{dining table}. Objects labeled as \textit{difficult} for object classification are not used in our experiments. 

For the experiments, we repeatedly sample sets of images containing one, two, and three categories. The training/validation set and testing set have the same distribution. For a single iteration, we sample 480 images for the training/validation set including 30 images with all labels, and 150 images each for sets containing zero, one, or two of the target labels. More than 5,000 images from the entire dataset are sampled at least once as we repeat the experiments with random samplings to compute statistical significance.   

%\paragraph{Microsoft COCO} The Microsoft COCO~\cite{MScoco} is a new image recognition, segmentation, and captioning dataset. It contains more than 70 categories, more than 300,000 images and around 5 captions per image. We use one of the most promising Frequent Itemset Mining methods, e.g Linear time Closed itemset Miner (LCM)~\cite{uno2004efficient} to find out the most common combination of \textit{some} categories in the images. We choose the most common combination of 6 labels in images which are: \textit{person}, \textit{cup}, \textit{fork}, \textit{knife}, \textit{chair} and \textit{dining table}. 

%We sampled the images as $k$-positive images ($k=0,1,2,\cdots,6$) have equally amount in training/validation set or in testing set. For example, in the experiments, we randomly sample 150 images for each $k$-positive images for training/validation, and 100 images for each for testing. As more random sampling experiments are carried out further, around 12,000 images in total have been used from the entire Microsoft COCO dataset.

%\subsection{Method}
\paragraph{Feature Extraction}
We use Overfeat~\cite{overfeat} to extract image features. Overfeat has been trained for the image classification task on ImageNet ILSVRC 2013, and has achieved good performance on a range of image classification problems including the PASCAL VOC dataset~\cite{kthCNN}.

Following \cite{kthCNN} we use the fully connected layer (layer 22) of the network. All images from the datasets are first resized to $221\times221$ before the feature extraction. Overfeat then gives a feature vector of 4096 dimensions. The feature vector is further signed power normalized and $\ell_2$ normalized. Then we replicate the feature vector to form an instance  $x_i \in \mathbb{R}^{p\times 4096}$ for the input to the classifiers, where $p$ is the number of labels taken in to account for the task. %\todo{If short on space, this paragraph can be replaced with: We have followed the feature extraction pipeline described in~\cite{kthCNN}.} 

\paragraph{Submodular Losses} In this task, we first define the submodular loss function as follows:
\begin{equation}
\Delta(y,\tilde{y}):=\min\left(l_{\textrm{max}}, \left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle \right)\label{eq:vocsubloss}
\end{equation}
where $\odot$ is the Hadamard product, 
%$\mathbf{I}=\{j|y^j\neq\tilde{y}^j\}$ gives the set of incorrect prediction labels, $\operatorname{Ind}(\mathbf{I})$ gives the binary index vector of set $\mathbf{I}$, 
$l_{\textrm{max}}$ is the maximal risk value, $\beta >0$ is a coefficient vector of size $p$ that accounts for the relative importance of each category label. $l_{max} < \| \beta \|_1$ ensures the function is strictly submodular. %$I$ gives the indicator vector of $y\neq\tilde{y}$. 
This function is an analogue to the submodular increasing function in Sec.~\ref{sec:visual}. In the VOC experiments, we order the category labels as \textit{person}, \textit{dining table} and \textit{chair}. We set $l_{\textrm{max}}=1.3$ and $\beta = [1\ 0.5\ 0.2]$. The empirical results with this submodular loss are shown in Table~\ref{tab:lossvoc} and Fig.~\ref{fig:gapTOY}.

We have carried out experiments with another submodular loss function:
\begin{equation}\label{eq:mixsubloss}
\Delta(y,\tilde{y}):=1-\exp\left(-| \mathbf{I} |\right)+\left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle
\end{equation}
where $\mathbf{I}$ is the set of mispredicted labels.
The first part, $1-\exp\left(-|\mathbf{I}|\right)$, is a concave function depending only on the size of $\mathbf{I}$, as a consequence it is a submodular function; the second part is a modular function that penalizes labels proportionate to the coefficient vector  $\beta$ as above. The results with this submodular loss are shown in Table~\ref{tab:lossvoc2} and Fig.~\ref{fig:gapMIML}.  %which relative to the proportion of the positive samples in each category of the total training samples.
We additionally train and test with the 0-1 loss, which is equivalent to an SVM.

We compare different losses employed during training and during testing. %We then measure the empirical loss values as the average loss value for all images. 
$m_{sub}$ and $s_{sub}$ denote the use of the submodular loss with margin and slack rescaling, respectively. As this optimization is NP-hard, we have employed the approximate optimization procedure of~\cite{Nemhauser1978}.

\paragraph{Results}
We repeated each experiment 10 times with random sampling in order to obtain an estimate of the average performance.  
Table~\ref{tab:lossvoc} and Table~\ref{tab:lossvoc2} show the cross comparison of average loss values (with standard error) using different loss functions during training and during testing for the VOC dataset. %, using $l_{sub}$ as in Equation~\eqref{eq:vocsubloss} and in Equation~\eqref{eq:mixsubloss}, respectively.
As predicted by theory, training with the same loss function as used during testing yields the best results.  Slack and margin rescaling fail due to the necessity of approximate inference, which results in a poor discriminant function.  By contrast, the Lov\'{a}sz hinge yields the best performance when the submodular loss is used to evaluate the test predictions.  We do not expect that optimizing the submodular loss should give the best performance when the 0-1 loss is used to evaluate the test predictions.  Indeed in this case, the Lov\'{a}sz hinge trained on 0-1 loss corresponds with the best performing system.

Fig.~\ref{fig:gapTOY} and Fig.~\ref{fig:gapMIML} show for the two experiments the primal-dual gap as a function of the number of cutting-plane iterations using the Lov\'{a}sz hinge with submodular loss, as well as for a SVM (labeled 0-1), and margin and slack rescaling (labeled $m_{sub}$ and $s_{sub}$). This demonstrates that the empirical convergence of the Lov\'{a}sz hinge is at a rate comparable to an SVM, and is feasible to optimize in practice for real-world problems.

%%%%%%%%%%%%%%%%%%%%%% table for VOC %%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{testing loss} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $l_{sub}$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{training loss}}}
 & $l_{sub}$ &	$\mathbf{0.4371 \pm 0.0045}$  &  0.9329$\pm$0.0097  \\
 & 0-1       &	0.5091$\pm$0.0023             &  $\mathbf{0.8320 \pm 0.0074}$  \\
 & $s_{sub}$ &	0.4927$\pm$0.0067             &  0.8731$\pm$0.0073  \\
 & $m_{sub}$ &	0.4437$\pm$0.0034             &  1.0010$\pm$0.0080  \\
\hline
\end{tabular}
\caption{The cross comparison of average loss values (with standard error) using different loss functions during training and during testing. $l_{sub}$ is as in Equation~\eqref{eq:vocsubloss}. %As predicted by theory, 
Training with the same loss function as used during testing yields the best results.  Slack and margin rescaling fail due to the necessity of approximate inference, which results in a poor discriminant function.  The Lov\'{a}sz hinge trained on the appropriate loss yields the best performance in both cases.
}\label{tab:lossvoc}
\end{table}

\begin{table}[ht]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{testing loss} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $l_{sub}$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{training loss}}}
 & $l_{sub}$ &	$\mathbf{0.9447 \pm 0.0069}$  &  0.8786$\pm$0.0077  \\
 & 0-1       &	0.9877$\pm$0.0044             &  $\mathbf{0.8173 \pm 0.0061}$  \\
 & $s_{sub}$ &	0.9784$\pm$0.0052              &  0.8337$\pm$0.0054  \\
 & $m_{sub}$ &	0.9718$\pm$0.0041              &  0.9425$\pm$0.0054  \\
\hline
\end{tabular}
\caption{The cross comparison of average loss values (with standard error) using different loss functions during training and during testing. $l_{sub}$ is as in Equation~\eqref{eq:mixsubloss} (cf.\ comments for Table.~\ref{tab:lossvoc}).}\label{tab:lossvoc2}
\end{table}

%%%%%%%%%%%%%%%%%%%% figures of gap %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering
\subfigure{\label{fig:gapTOY}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ ]
{\includegraphics[width=0.45\linewidth]{gapVOC}}}
\subfigure{\label{fig:gapMIML}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[width=0.45\linewidth]{gapVOC2}}}
\caption{The primal-dual gap as a function of the number of cutting-plane iterations using the Lov\'{a}sz hinge with submodular loss, a SVM (labeled 0-1), and margin and slack rescaling with greedy inference (labeled $m_{sub}$ and $s_{sub}$). Fig.~\ref{fig:gapTOY} for the experiment using Equation~\eqref{eq:vocsubloss} and Fig.~\ref{fig:gapMIML} for Equation~\eqref{eq:mixsubloss}. This demonstrates that empirical convergence of the Lov\'{a}sz hinge is at a rate comparable to an SVM, and is feasible to optimize in practice for real-world problems.
}\label{fig:gap}
\end{figure}


==> ResultsArXiv.tex <==
\section{Experimental Results}\label{sec:Results}

We validate the Lov\'{a}sz hinge on a number of different experimental settings.  In Section~\ref{sec:Toy}, we demonstrate a synthetic problem motivated by an early detection task.  Next, we show that the Lov\'{a}sz hinge can be employed to improve image classification measured by the Jaccard loss on the PASCAL VOC dataset in Section~\ref{sec:Jaccardexp}.  Multi-label prediction with submodular losses is demonstrated on the PASCAL VOC dataset in Section~\ref{sec:PASCALmultilabelexp}, and on the MS COCO dataset in Section~\ref{sec:MSCOCOmultilabelexp}.  A summary of results is given in Section~\ref{sec:resultsSummary}.

\subsection{A Synthetic Problem}\label{sec:Toy}

We designed a synthetic problem motivated by early detection in a sequence of observations. As shown in Fig.~\ref{fig:toy}, each star represents one sample in a \textit{bag} and $p=15$ samples form one bag. %Our problem is based on the unit of bags (patterns). 
In each bag, the samples are arranged in a chronological order, with samples appearing earlier drawn from a different distribution than later samples. The red and magenta dots represent the early and late positive samples, respectively. The blue dots represent the negative samples. For the negative samples, there is no change in distribution between early and late samples, while the distribution of positive samples changes with time (e.g.\ as in the evolution of cancer from early to late stage).

We define the loss function as
\begin{equation}\label{eq:synthSubmodLoss}
\Delta_1(y,\tilde{y})=\sum_{i=1}^p\gamma_i l_{sub}(\mathbf{I}_i)
\end{equation}
where $\mathbf{I}_i=\{j| j \leq i, \tilde{y}^{j}\neq y^{j}\}$. Let $\gamma_i:=e^{-i} \ \forall i$. By this formulation, we penalize early mispredictions more than late mispredictions.  This is a realistic setting in many situations where, e.g.\ early detection of a disease leads to better patient outcomes. %If we set other values for $\gamma_i$, e.g $\gamma_i = 1-\frac{i}{p}$, we can further adjust the rate of early penalization. 
The loss $l_{sub}$ measures the misprediction rate up to the current time while being limited by an upper bound:
\begin{align}
\label{eq:subloss}
&l_{sub}(\mathbf{I}_i):=\min\left( | \mathbf{I}_i |,\ \frac{i}{2}\right) .
\end{align}
As $\Delta$ is a positively weighted sum of submodular losses, it is submodular.
We additionally train and test with the 0-1 loss, which is equivalent to an SVM and Hamming loss in the Lov\'{a}sz hinge.
We use different losses during training and during testing, then we measure the empirical loss values of one prediction as the average loss value for all images shown in Table.~\ref{tab:lossToy}.  We have trained on 1000 bags and tested on 5000 bags.
$\mathbf{M}$ and $\mathbf{S}$ denote the use of the submodular loss with margin and slack rescaling, respectively. As this optimization is intractable, we have employed the approximate optimization procedure of~\cite{Nemhauser1978}.

As predicted by theory, training with the same loss function as used during testing yields the best results.  Slack and margin rescaling fail due to the necessity of approximate inference, which results in a poor discriminant function.  By contrast, the Lov\'{a}sz hinge yields the best performance on the submodular loss.
\begin{figure}
\begin{minipage}{0.45\textwidth}
%%%%%%%%%%%%%%%%% examples of images %%%%%%%%%%%%%%%%%%
\centering
\includegraphics[width=.75\textwidth]{Toy_lastMinuteNewMark-crop.pdf}
\caption{\label{fig:toy} The disributions of samples for a synthetic binary classification problem motivated by the problem of early detection in a temporal sequence.  As in, e.g.\ disease evolution, the distribution of early stage samples differs from that of late stage samples. }	
\end{minipage}
\begin{minipage}{0.49\textwidth}
%%%%%%%%%%%%%%%%%%%%%% table for toy problem %%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}[!t]\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{Test} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $\Delta_1$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{Train}}}
 & $\mathbf{L}$ &	$\mathbf{0.100 \pm 0.001}$  &  7.42$\pm$0.01  \\
 & 0-1   &	0.166$\pm$0.001  &  $\mathbf{2.87 \pm 0.02}$  \\
 & $\mathbf{S}$ &	0.144$\pm$0.001  &  7.69$\pm$0.01  \\
 & $\mathbf{M}$ &	0.154$\pm$0.001  &  3.01$\pm$0.01  \\
\hline
\end{tabular}}
\captionof{table}{\label{tab:lossToy}For the synthetic problem, the cross comparison of average loss values (with standard error) using different convex surrogates for submodular loss in Equation~\eqref{eq:synthSubmodLoss} during training, 0-1 loss for comparison, and testing with different losses.}
%\end{table}
\end{minipage}
\end{figure}

\subsection{PASCAL VOC image classification}\label{sec:Jaccardexp}
We consider an image classification task on the Pascal VOC dataset~\cite{pascal-voc-2007}.  This challenging dataset contains around 10,000 images of 20 classes including animals, handmade and natural objects such as \textit{person}, \textit{bird}, \textit{aeroplane} etc. In the training set, which contains 5,011 images of different categories, the number of positive samples varies largely, we evaluate the prediction on the entire training/testing set with the Jaccard loss as in Equation~\eqref{eq:jaccard}.

We use Overfeat~\cite{overfeat} to extract image features following the procedure described in~\cite{kthCNN}. Overfeat has been trained for the image classification task on ImageNet ILSVRC 2013, and has achieved good performance on a range of image classification problems.

We compare learning with the Taccard loss with the Lov\'{a}sz hinge with learning an SVM (labeled 0-1 in the results tables). The empirical error values using different loss function during test time are shown in Table~\ref{tab:jaccarderrors}. %The average precision values are shown in Table~\ref{tab:jaccardaps}.

\begin{table*}[!t]\centering
\resizebox{1.25\linewidth}{!}{
\begin{tabular}{ll*{20}{c}}
\hline
\multicolumn{2}{c|}{}  & \multicolumn{2}{|c}{aeroplane} & \multicolumn{2}{|c}{bicycle} & \multicolumn{2}{|c}{bird} & \multicolumn{2}{|c}{boat} & \multicolumn{2}{|c}{bottle} & \multicolumn{2}{|c}{bus} & \multicolumn{2}{|c}{car} & \multicolumn{2}{|c}{cat} & \multicolumn{2}{|c}{chair} & \multicolumn{2}{|c}{cow} \\
\multicolumn{2}{c|}{Test time} & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ &  0-1   \\
\hline
\multirow{2}{*}{\rotatebox{90}{Train}}
 & \multicolumn{1}{r|}{$\mathbf{L}$}   & $0.310$ & \multicolumn{1}{r|}{$0.014$}  & $0.436$ & \multicolumn{1}{r|}{$0.025$}  & $0.371$ & \multicolumn{1}{r|}{$0.025$}  & $0.416$ & \multicolumn{1}{r|}{$0.017$}  & $0.761$ & \multicolumn{1}{r|}{$0.062$}  & $0.539$ & \multicolumn{1}{r|}{$0.026$}  & $0.399$ & \multicolumn{1}{r|}{$0.076$}  & $0.426$ & \multicolumn{1}{r|}{$0.035$}  & $0.687$ & \multicolumn{1}{r|}{$0.121$}  & $0.640$ & $0.027$ \\  
 & \multicolumn{1}{r|}{0-1}     & $0.310$ & \multicolumn{1}{r|}{$0.014$}  & $0.466$ & \multicolumn{1}{r|}{$0.027$}  & $0.399$ & \multicolumn{1}{r|}{$0.025$}  & $0.483$ & \multicolumn{1}{r|}{$0.020$}  & $0.917$ & \multicolumn{1}{r|}{$0.045$}  & $0.661$ & \multicolumn{1}{r|}{$0.025$}  & $0.397$ & \multicolumn{1}{r|}{$0.068$}  & $0.469$ & \multicolumn{1}{r|}{$0.034$}  & $0.744$ & \multicolumn{1}{r|}{$0.090$}  & $0.892$ & $0.023$  \\
 \hline 
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{diningtable} & \multicolumn{2}{|c}{dog} & \multicolumn{2}{|c}{horse} & \multicolumn{2}{|c}{motorbike} & \multicolumn{2}{|c}{person} & \multicolumn{2}{|c}{pottedplant} & \multicolumn{2}{|c}{sheep} & \multicolumn{2}{|c}{sofa} & \multicolumn{2}{|c}{train} & \multicolumn{2}{|c}{tvmonitor}\\
\multicolumn{2}{c|}{Test time} & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ & \multicolumn{1}{r|}{0-1}  & $\Delta_J$ &  0-1 \\
\hline
\multirow{2}{*}{\rotatebox{90}{Train}}
 & \multicolumn{1}{r|}{$\mathbf{L}$}  & $0.664$ & \multicolumn{1}{r|}{$0.055$}  & $0.475$ & \multicolumn{1}{r|}{$0.054$}  & $0.405$ & \multicolumn{1}{r|}{$0.029$}  & $0.439$ & \multicolumn{1}{r|}{$0.025$}  & $0.347$ & \multicolumn{1}{r|}{$0.180$}  & $0.747$ & \multicolumn{1}{r|}{$0.058$}  & $0.580$ & \multicolumn{1}{r|}{$0.017$}  & $0.710$ & \multicolumn{1}{r|}{$0.062$}  & $0.306$ & \multicolumn{1}{r|}{$0.018$}  & $0.588$ & $0.042$  \\  
 & \multicolumn{1}{r|}{0-1}    & $0.695$ & \multicolumn{1}{r|}{$0.043$}  & $0.564$ & \multicolumn{1}{r|}{$0.050$}  & $0.451$ & \multicolumn{1}{r|}{$0.032$}  & $0.493$ & \multicolumn{1}{r|}{$0.027$}  & $0.325$ & \multicolumn{1}{r|}{$0.151$}  & $0.846$ & \multicolumn{1}{r|}{$0.043$}  & $0.611$ & \multicolumn{1}{r|}{$0.016$}  & $0.730$ & \multicolumn{1}{r|}{$0.062$}  & $0.325$ & \multicolumn{1}{r|}{$0.018$}  & $0.690$ & $0.036$ \\
 \hline 
\end{tabular}
}
\caption{\label{tab:jaccarderrors}For the VOC image classification task, the cross comparison of average loss values using the jaccard loss as well as 0-1 loss during training and during testing for the 20 categories.
}
\end{table*}

\subsection{PASCAL VOC multilabel prediction}\label{sec:PASCALmultilabelexp}
We consider next a multi-label prediction task on Pascal VOC dataset~\cite{pascal-voc-2007}, in which multiple labels need to be predicted simultaneously and for which a submodular loss over labels is to be minimized. Fig.~\ref{fig:voc} shows example images from the dataset, including three categories i.e.\ \textit{people}, \textit{tables} and \textit{chairs}. 
%Fig.\ref{fig:table} and Fig.\ref{fig:chair} contain all of these three categories/labels while Fig.\ref{fig:chaironly} contains only dining tables and chairs. 
If a subsequent prediction task focuses on detecting ``\textit{people sitting around a table}'', the initial multilabel prediction should emphasize that all labels must be correct \emph{within a given image}. This contrasts with a traditional multi-label prediction task in which a loss function decomposes over the individual predictions. The misprediction of a single label, e.g.\ \textit{person}, will preclude the chance to predict correctly the combination of all three labels. %The fact that the augmentation of mistakes doesn't make the prediction action equally worse. 
This corresponds exactly to the property of diminishing returns of a submodular function. 
 
While using classic modular losses such as 0-1 loss, the classifier is trained to minimize the sum of incorrect predictions, so the complex interaction between label mispredictions is not considered. In this work, we use a new submodular loss function and apply the Lov\'{a}sz hinge to enable efficient convex risk minimization.
\begin{figure}\centering
\subfigure{\label{fig:table}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.75in]{diningtable_04.jpg}}}
\subfigure{\label{fig:chair}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.75in]{chair_03.jpg}}}
\subfigure{\label{fig:chaironly}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.75in]{chair_01.jpg}}}
\caption{\label{fig:voc}Examples from the PASCAL VOC dataset. Fig.\ref{fig:table} and Fig.\ref{fig:chair} contain three categories: \textit{people}, \textit{table} and \textit{chair}. Fig.\ref{fig:chaironly} contains \textit{table} and \textit{chair}.}
\end{figure}
 In our work, we choose the most common combination of three categories: \textit{person}, \textit{chairs} and \textit{dining table}. Objects labeled as \textit{difficult} for object classification are not used in our experiments. 

For the experiments, we repeatedly sample sets of images containing one, two, and three categories. The training/validation set and testing set have the same distribution. For a single iteration, we sample 480 images for the training/validation set including 30 images with all labels, and 150 images each for sets containing zero, one, or two of the target labels. More than 5,000 images from the entire dataset are sampled at least once as we repeat the experiments with random samplings to compute statistical significance.   
In this task, we first define the submodular loss function as follows:
\begin{equation}
\Delta_2(y,\tilde{y}):=\min\left(l_{\textrm{max}}, \left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle \right)\label{eq:vocsubloss}
\end{equation}
where $\odot$ is the Hadamard product, 
%$\mathbf{I}=\{j|y^j\neq\tilde{y}^j\}$ gives the set of incorrect prediction labels, $\operatorname{Ind}(\mathbf{I})$ gives the binary index vector of set $\mathbf{I}$, 
$l_{\textrm{max}}$ is the maximal risk value, $\beta >0$ is a coefficient vector of size $p$ that accounts for the relative importance of each category label. $l_{max} < \| \beta \|_1$ ensures the function is strictly submodular. %$I$ gives the indicator vector of $y\neq\tilde{y}$. 
This function is an analogue to the submodular increasing function in Sec.~\ref{sec:visual}. In the VOC experiments, we order the category labels as \textit{person}, \textit{dining table} and \textit{chair}. We set $l_{\textrm{max}}=1.3$ and $\beta = [1\ 0.5\ 0.2]$. 

We have additionally carried out experiments with another submodular loss function:
\begin{equation}\label{eq:mixsubloss}
\Delta_3(y,\tilde{y}):=1-\exp\left(-| \mathbf{I} |\right)+\left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle
\end{equation}
where $\mathbf{I}$ is the set of mispredicted labels.
The first part, $1-\exp\left(-|\mathbf{I}|\right)$, is a concave function depending only on the size of $\mathbf{I}$, as a consequence it is a submodular function; the second part is a modular function that penalizes labels proportionate to the coefficient vector  $\beta$ as above. The results with this submodular loss are shown in Table~\ref{tab:lossvoc} .  %which relative to the proportion of the positive samples in each category of the total training samples.
We additionally train and test with the 0-1 loss, which is equivalent to an SVM.

We compare different losses employed during training and during testing. %We then measure the empirical loss values as the average loss value for all images. 
$\mathbf{M}$ and $\mathbf{S}$ denote the use of the submodular loss with margin and slack rescaling, respectively. The empirical results with this submodular loss are shown in Table~\ref{tab:lossvoc}.

%%%%%%%%%%%%%%%%%%%%%% table for VOC %%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{Test} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $\Delta_2$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{Train}}}
 & $\mathbf{L}$ &	$\mathbf{0.4371 \pm 0.0045}$  &  0.9329$\pm$0.0097  \\
 & 0-1       &	0.5091$\pm$0.0023             &  $\mathbf{0.8320 \pm 0.0074}$  \\
 & $\mathbf{S}$ &	0.4927$\pm$0.0067             &  0.8731$\pm$0.0073  \\
 & $\mathbf{M}$ &	0.4437$\pm$0.0034             &  1.0010$\pm$0.0080  \\
\hline
\end{tabular}
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{Test} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $\Delta_3$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{Train}}}
 & $\mathbf{L}$ &	$\mathbf{0.9447 \pm 0.0069}$  &  0.8786$\pm$0.0077  \\
 & 0-1       &	0.9877$\pm$0.0044             &  $\mathbf{0.8173 \pm 0.0061}$  \\
 & $\mathbf{S}$ &	0.9784$\pm$0.0052              &  0.8337$\pm$0.0054  \\
 & $\mathbf{M}$ &	0.9718$\pm$0.0041              &  0.9425$\pm$0.0054  \\
\hline
\end{tabular}
\caption{\label{tab:lossvoc}For the VOC multilabel prediction task, the cross comparison of average loss values (with standard error) using submodular loss as in Equation~\eqref{eq:vocsubloss} and Equation~\eqref{eq:mixsubloss}, as well as 0-1 loss during training and during testing.}
\end{table*}

\subsection{Microsoft COCO multilabel prediction}\label{sec:MSCOCOmultilabelexp}
In this section, we consider the multi-label prediction task on Microsoft COCO dataset. On detecting a \emph{dinner scene}, the initial multi-label prediction should emphasize that all labels must be correct \emph{within a given image}, while MS COCO provides more relating categories e.g.~\emph{people}, \emph{dinning tables}, \emph{forks} or \emph{cups}. 
Submodular loss functions coincides with the fact that misprediction of a single label, e.g.\ \emph{person}, will preclude the chance to predict correctly the combination of all labels. 
Fig.~\ref{fig:coco} shows example images from the Microsoft COCO dataset~\cite{MScoco}.

\begin{figure} \centering
\subfigure{\label{fig:coco1}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.75in]{COCO0110.jpg}}}
\subfigure{\label{fig:coco2}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.75in]{COCO4719.jpg}}}
\subfigure{\label{fig:coco3}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.75in]{COCO2459.jpg}}}
\caption{\label{fig:coco} Examples from the Microsoft COCO dataset. Fig.~\ref{fig:coco1} contains all the categories of interest (cf.\ Section~\ref{sec:Results}); Fig.~\ref{fig:coco2} contains \emph{dining table}, \emph{fork} and \emph{cup}; Fig.~\ref{fig:coco3} is not a dining scene but contains \emph{people}. }
\end{figure}

%\paragraph{Microsoft COCO}
The Microsoft COCO dataset~\cite{MScoco} is an image recognition, segmentation, and captioning dataset. It contains more than 70 categories, more than 300,000 images and around 5 captions per image. \mycorr{We have used frequent itemset mining~\cite{uno2004efficient} to determine the most common combination of categories in an image. For sets of size 6, these are: \emph{person}, \emph{cup}, \emph{fork}, \emph{knife}, \emph{chair} and \emph{dining table}. }

For the experiments, we repeatedly sample sets of images containing $k$ ($k=0,1,2,\cdots,6$)  categories. The training/validation set and testing set have the same distribution. For a single iteration, we sample 1050 images for the training/validation set including 150 images each for sets containing $k$ ($k=0,1,2,\cdots,6$) of the target labels. More than 12,000 images from the entire dataset are sampled at least once as we repeat the experiments to compute statistical significance.  

%\paragraph{Submodular Losses} 
In this task, we first use a submodular loss function as follows:
\begin{equation}
%\Delta(y,\tilde{y}):=\min\left(l_{\textrm{max}}, \left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle \right)\label{eq:vocsubloss}
\Delta_4(y,\tilde{y}):=1-\exp\left(-\alpha| \mathbf{I} |\right)\label{eq:cocosubloss}
\end{equation}
where $\mathbf{I}$ is the set of mispredicted labels. $1-\exp\left(-|\mathbf{I}|\right)$, is a concave function depending only on the size of $\mathbf{I}$, as a consequence it is a submodular function, $\alpha$ is a positive coefficient that effect the increasing rate of the concave function thus the submodularity of the set function. In the experiment we set $\alpha=1$.
%$\mathbf{I}=\{j|y^j\neq\tilde{y}^j\}$ gives the set of incorrect prediction labels, $\operatorname{Ind}(\mathbf{I})$ gives the binary index vector of set $\mathbf{I}$, 
%$l_{\textrm{max}}$ is the maximal risk value, $\beta $ is a coefficient vector of size $p$ that accounts for the relative importance of each category label. $l_{max} < \| \beta \|_1$ ensures the function is strictly submodular. %$I$ gives the indicator vector of $y\neq\tilde{y}$. 
%This function is an analogue to the submodular increasing function in Sec.~\ref{sec:visual}. 
 and Fig.~\ref{fig:gapTOY}.

We have also carried out experiments with the submodular loss function used in VOC experiments:
\begin{equation}\label{eq:cocosubloss2}
\Delta_5(y,\tilde{y}):=1-\exp\left(-| \mathbf{I} |\right)+\left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle
\end{equation}
\mycorr{where we set $\beta = [1\ 0.8\ 0.7\ 0.6\ 0.5\ 0.4]^{T}$ according to the size of the object that we order the category labels as \emph{person}, \emph{dining table}, \emph{chair}, \emph{cup}, \emph{fork} and \emph{knife}.} 
 % and Fig.~\ref{fig:gapMIML}.  %which relative to the proportion of the positive samples in each category of the total training samples.
We also train and test with the 0-1 loss, which is equivalent to an SVM.

We compare different losses employed during training and during testing. %We then measure the empirical loss values as the average loss value for all images. 
$\mathbf{M}$ and $\mathbf{S}$ denote the use of the submodular loss with margin and slack rescaling, respectively. As this optimization is NP-hard, we have employed %the approximate optimization procedure of~\cite{Nemhauser1978}.
\mycorr{the simple application of the greedy approach as is common in (non-monotone) submodular maximization (e.g.~\cite{krause2012survey}).}
%\paragraph{Results}

We repeated each experiment 10 times with random sampling in order to obtain an estimate of the average performance.  
Table~\ref{tab:losscoco} show the cross comparison of average loss values (with standard error) using different loss functions during training and during testing for the COCO dataset. %, using $l_{sub}$ as in Equation~\eqref{eq:vocsubloss} and in Equation~\eqref{eq:mixsubloss}, respectively.

\subsection{Empirical Results}\label{sec:resultsSummary}
From the empirical results in Table~\ref{tab:lossToy}, Table~\ref{tab:jaccarderrors}, Table~\ref{tab:lossvoc} and Table~\ref{tab:losscoco}, we can see that training with the same submodular loss functions as used during testing yields the best results.  Slack and margin rescaling fail due to the necessity of approximate inference, which results in a poor discriminant function.  By contrast, the Lov\'{a}sz hinge yields the best performance when the submodular loss is used to evaluate the test predictions.  We do not expect that optimizing the submodular loss should give the best performance when the 0-1 loss is used to evaluate the test predictions.  Indeed in this case, the Lov\'{a}sz hinge trained on 0-1 loss corresponds with the best performing system.

Fig.~\ref{fig:gapTOY} and Fig.~\ref{fig:gapMIML} show for the two submodular functions the primal-dual gap as a function of the number of cutting-plane iterations using the Lov\'{a}sz hinge with submodular loss, as well as for a SVM (labeled 0-1), and margin and slack rescaling (labeled $\mathbf{M}$ and $\mathbf{S}$). This demonstrates that the empirical convergence of the Lov\'{a}sz hinge is at a rate comparable to an SVM, and is feasible to optimize in practice for real-world problems.
%%%%%%%%%%%%%%%%%%%%%% table for COCO %%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{Test} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $\Delta_4$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{Train}}}
 & $\mathbf{L}$ &	$\mathbf{0.5567 \pm 0.0057}$  &  1.4295$\pm$0.0194  \\
 & 0-1       &	0.5729$\pm$0.0060             &  $\mathbf{1.3924 \pm 0.0195}$  \\
 & $\mathbf{S}$ &	0.5875$\pm$0.0065             &  1.4940$\pm$0.0233  \\
 & $\mathbf{M}$ &	0.5820$\pm$0.0063             &  1.4802$\pm$0.0233  \\
\hline
\end{tabular}
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{Test} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $\Delta_5$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{Train}}}
 & $\mathbf{L}$ &	$\mathbf{1.3767 \pm 0.0143}$  &  1.3003$\pm$0.0176  \\
 & 0-1       &	1.3813$\pm$0.0135             &  $\mathbf{1.2975 \pm 0.0152}$  \\
 & $\mathbf{S}$ &	1.4711$\pm$0.0153             &  1.3832$\pm$0.0156  \\
 & $\mathbf{M}$ &	1.4811$\pm$0.0117             &  1.4016$\pm$0.0136  \\
\hline
\end{tabular}
\caption{\label{tab:losscoco}For the MS COCO prediction task, the comparison of average loss values (with standard error) using submodular loss  as in Equation~\eqref{eq:cocosubloss} and Equation~\eqref{eq:cocosubloss2}, as well as 0-1 loss during training and during testing.}\label{tab:losscoco}
\end{table*}

%%%%%%%%%%%%%%%%%%%% figures of gap %%%%%%%%%%%%%%%%%%%%
\begin{figure*}\centering
\subfigure{\label{fig:gapTOY}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ ]
{\includegraphics[width=0.45\linewidth]{gapCOCO1.pdf}}}
\subfigure{\label{fig:gapMIML}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[width=0.45\linewidth]{gapCOCO3.pdf}}}
\caption{The primal-dual gap as a function of the number of cutting-plane iterations using the Lov\'{a}sz hinge with submodular loss, a SVM (labeled 0-1), and margin and slack rescaling with greedy inference (labeled $m_{sub}$ and $s_{sub}$). Fig.~\ref{fig:gapTOY} for the experiment using Equation~\eqref{eq:cocosubloss} and Fig.~\ref{fig:gapMIML} for Equation~\eqref{eq:cocosubloss2}. This demonstrates that empirical convergence of the Lov\'{a}sz hinge is at a rate comparable to an SVM, and is feasible to optimize in practice for real-world problems.
}\label{fig:gap}
\end{figure*}


==> Results_save.tex <==
\section{Experimental Results}\label{sec:Results}
%\subsection{PASCAL VOC}
In this section, we consider a task in which multiple labels need to be predicted simultaneously and for which a submodular loss over labels is to be minimized.\footnote{Additional prediction tasks are demonstrated in the supplementary material due to space constraints.} 
%Fig.~\ref{fig:voc} shows example images from the Pascal VOC dataset~\cite{pascal-voc-2007}, which include \textit{people}, \textit{tables} or \textit{chairs}. 
%Fig.\ref{fig:table} and Fig.\ref{fig:chair} contain all of these three categories/labels while Fig.\ref{fig:chaironly} contains only dining tables and chairs. 
If a subsequent prediction task focuses on detecting \mycorr{a \emph{dinner scene}}, the initial multilabel prediction should emphasize that all labels \mycorr{e.g.\emph{people}, \emph{dinning tables}, \emph{forks} or \emph{knif}} must be correct \emph{within a given image}. This contrasts with a traditional multi-label prediction task in which a loss function decomposes over the individual predictions. The misprediction of a single label, e.g.\ \emph{person}, will preclude the chance to predict correctly the combination of all three labels. %The fact that the augmentation of mistakes doesn't make the prediction action equally worse. 
This corresponds exactly to the property of diminishing returns of a submodular function. 
\mycorr{Fig.~\ref{fig:coco} shows example images from the Microsoft COCO dataset~\cite{MScoco}.}

While using classic modular losses such as 0-1 loss, the classifier is trained to minimize the sum of incorrect predictions, so the complex interaction between label mispredictions is not considered. In this work, we use a new submodular loss function and apply the Lov\'{a}sz hinge to enable efficient convex risk minimization.
\begin{figure}[t]  \centering
\subfigure{\label{fig:table}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.65in]{COCO0110}}}
\subfigure{\label{fig:chair}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.65in]{COCO4719}}}
\subfigure{\label{fig:chaironly}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[height=0.65in]{COCO2459}}}
\caption{\label{fig:coco}Examples from the Microsoft COCO dataset. Fig.\ref{fig:table} contains all the categories of interest; Fig.\ref{fig:chair} contains \emph{dining table}, \emph{fork} and \emph{cup}; Fig.\ref{fig:chaironly} is not a dining scene but contains \emph{people}.}
\end{figure}
\iffalse
\paragraph{PASCAL VOC dataset} We use the PASCAL VOC~\cite{pascal-voc-2007} dataset for this prediction task. This challenging dataset contains around 10,000 images of 20 classes including animals, handmade and natural objects. In our work, we choose the most common combination of three categories: \textit{person}, \textit{chairs} and \textit{dining table}. Objects labeled as \textit{difficult} for object classification are not used in our experiments. 

For the experiments, we repeatedly sample sets of images containing one, two, and three categories. The training/validation set and testing set have the same distribution. For a single iteration, we sample 480 images for the training/validation set including 30 images with all labels, and 150 images each for sets containing zero, one, or two of the target labels. More than 5,000 images from the entire dataset are sampled at least once as we repeat the experiments with random samplings to compute statistical significance.   \fi

\paragraph{Microsoft COCO}
The Microsoft COCO~\cite{MScoco} is a new image recognition, segmentation, and captioning dataset. It contains more than 70 categories, more than 300,000 images and around 5 captions per image. \mycorr{We use one of the most promising Frequent Itemset Mining methods, e.g Linear time Closed itemset Miner (LCM)~\cite{uno2004efficient} to find out the most common combination of \emph{some} categories in the images. We choose the most common combination of 6 labels in images which are: \emph{person}, \emph{cup}, \emph{fork}, \emph{knife}, \emph{chair} and \emph{dining table}. }

For the experiments, we repeatedly sample sets of images containing \mycorr{$k$ ($k=0,1,2,\cdots,6$)} categories. The training/validation set and testing set have the same distribution. For a single iteration, we sample 1050 images for the training/validation set including 150 images each for sets containing $k$ ($k=0,1,2,\cdots,6$) of the target labels. More than 12,000 images from the entire dataset are sampled at least once as we repeat the experiments with random samplings to compute statistical significance.  

%\subsection{Method}
\paragraph{Feature Extraction}
We use Overfeat~\cite{overfeat} to extract image features. Overfeat has been trained for the image classification task on ImageNet ILSVRC 2013, and has achieved good performance on a range of image classification problems including the Microsoft COCO dataset~\citep{kthCNN}.

Following \cite{kthCNN} we use the fully connected layer (layer 22) of the network. All images from the datasets are first resized to $221\times221$ before the feature extraction. Overfeat then gives a feature vector of 4096 dimensions. The feature vector is further signed power normalized and $\ell_2$ normalized. Then we replicate the feature vector to form an instance  $x_i \in \mathbb{R}^{p\times 4096}$ for the input to the classifiers, where $p$ is the number of labels taken in to account for the task. %\todo{If short on space, this paragraph can be replaced with: We have followed the feature extraction pipeline described in~\cite{kthCNN}.} 

\paragraph{Submodular Losses} In this task, we first define the submodular loss function as follows:
\begin{equation}
%\Delta(y,\tilde{y}):=\min\left(l_{\textrm{max}}, \left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle \right)\label{eq:vocsubloss}
\mycorr{\Delta(y,\tilde{y}):=1-\exp\left(-| \mathbf{I} |\right) \label{eq:vocsubloss}}
\end{equation}
where $\odot$ is the Hadamard product, 
%$\mathbf{I}=\{j|y^j\neq\tilde{y}^j\}$ gives the set of incorrect prediction labels, $\operatorname{Ind}(\mathbf{I})$ gives the binary index vector of set $\mathbf{I}$, 
$l_{\textrm{max}}$ is the maximal risk value, $\beta >0$ is a coefficient vector of size $p$ that accounts for the relative importance of each category label. $l_{max} < \| \beta \|_1$ ensures the function is strictly submodular. %$I$ gives the indicator vector of $y\neq\tilde{y}$. 
This function is an analogue to the submodular increasing function in Sec.~\ref{sec:visual}. \mycorr{In the experiments, we order the category labels as \emph{person}, \emph{cup}, \emph{fork}, \emph{knife}, \emph{chair} and \emph{dining table}. We set $l_{\textrm{max}}=2.0$ and $\beta = [1\ 0.6\ 0.5\ 0.4\ 0.7\ 0.8]$.} The empirical results with this submodular loss are shown in Table~\ref{tab:lossvoc} and Fig.~\ref{fig:gapTOY}.

We have carried out experiments with another submodular loss function:
\begin{equation}\label{eq:mixsubloss}
\Delta(y,\tilde{y}):=1-\exp\left(-| \mathbf{I} |\right)+\left\langle \beta, (1-y \odot \tilde{y}) / 2 \right\rangle
\end{equation}
where $\mathbf{I}$ is the set of mispredicted labels.
The first part, $1-\exp\left(-|\mathbf{I}|\right)$, is a concave function depending only on the size of $\mathbf{I}$, as a consequence it is a submodular function; the second part is a modular function that penalizes labels proportionate to the coefficient vector  $\beta$ as above. The results with this submodular loss are shown in Table~\ref{tab:lossvoc2} and Fig.~\ref{fig:gapMIML}.  %which relative to the proportion of the positive samples in each category of the total training samples.
We additionally train and test with the 0-1 loss, which is equivalent to an SVM.

We compare different losses employed during training and during testing. %We then measure the empirical loss values as the average loss value for all images. 
$m_{sub}$ and $s_{sub}$ denote the use of the submodular loss with margin and slack rescaling, respectively. As this optimization is NP-hard, we have employed %the approximate optimization procedure of~\cite{Nemhauser1978}.
\mycorr{the simple application of the greedy approach as is common in (non-monotone) submodular maximization (e.g. ~\cite{krause2012survey}).}
\paragraph{Results}
We repeated each experiment 10 times with random sampling in order to obtain an estimate of the average performance.  
Table~\ref{tab:lossvoc} and Table~\ref{tab:lossvoc2} show the cross comparison of average loss values (with standard error) using different loss functions during training and during testing for the VOC dataset. %, using $l_{sub}$ as in Equation~\eqref{eq:vocsubloss} and in Equation~\eqref{eq:mixsubloss}, respectively.
As predicted by theory, training with the same loss function as used during testing yields the best results.  Slack and margin rescaling fail due to the necessity of approximate inference, which results in a poor discriminant function.  By contrast, the Lov\'{a}sz hinge yields the best performance when the submodular loss is used to evaluate the test predictions.  We do not expect that optimizing the submodular loss should give the best performance when the 0-1 loss is used to evaluate the test predictions.  Indeed in this case, the Lov\'{a}sz hinge trained on 0-1 loss corresponds with the best performing system.

Fig.~\ref{fig:gapTOY} and Fig.~\ref{fig:gapMIML} show for the two experiments the primal-dual gap as a function of the number of cutting-plane iterations using the Lov\'{a}sz hinge with submodular loss, as well as for a SVM (labeled 0-1), and margin and slack rescaling (labeled $m_{sub}$ and $s_{sub}$). This demonstrates that the empirical convergence of the Lov\'{a}sz hinge is at a rate comparable to an SVM, and is feasible to optimize in practice for real-world problems.
%%%%%%%%%%%%%%%%%%%%%% table for VOC %%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{testing loss} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $l_{sub}$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{training loss}}}
 & $l_{sub}$ &	$\mathbf{0.7908 \pm 0.0113}$  &  1.3035$\pm$0.0182  \\
 & 0-1       &	0.7941$\pm$0.0102             &  $\mathbf{1.2863 \pm 0.0175}$  \\
 & $s_{sub}$ &	0.8739$\pm$0.0133             &  1.4397$\pm$0.0219  \\
 & $m_{sub}$ &	0.8722$\pm$0.0115             &  1.4365$\pm$0.0206  \\
\hline
\end{tabular}
\caption{The cross comparison of average loss values (with standard error) using different loss functions during training and during testing. $l_{sub}$ is as in Equation~\eqref{eq:vocsubloss}. %As predicted by theory, 
Training with the same loss function as used during testing yields the best results.  Slack and margin rescaling fail due to the necessity of approximate inference, which results in a poor discriminant function.  The Lov\'{a}sz hinge trained on the appropriate loss yields the best performance in both cases.
}\label{tab:lossvoc}
\end{table}
\begin{table}[ht]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{testing loss} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $l_{sub}$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{training loss}}}
 & $l_{sub}$ &	$\mathbf{1.3767 \pm 0.0143}$  &  1.3003$\pm$0.0176  \\
 & 0-1       &	1.3813$\pm$0.0135             &  $\mathbf{1.2975 \pm 0.0152}$  \\
 & $s_{sub}$ &	1.4711$\pm$0.0153             &  1.3832$\pm$0.0156  \\
 & $m_{sub}$ &	1.4811$\pm$0.0117             &  1.4016$\pm$0.0136  \\
\hline
\end{tabular}
\caption{The cross comparison of average loss values (with standard error) using different loss functions during training and during testing. $l_{sub}$ is as in Equation~\eqref{eq:mixsubloss} (cf.\ comments for Table.~\ref{tab:lossvoc}).}\label{tab:lossvoc2}
\end{table}

\iffalse
%%%%%%%%%%%%%%%%%%%%%% table for VOC %%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{testing loss} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $l_{sub}$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{training loss}}}
 & $l_{sub}$ &	$\mathbf{0.4371 \pm 0.0045}$  &  0.9329$\pm$0.0097  \\
 & 0-1       &	0.5091$\pm$0.0023             &  $\mathbf{0.8320 \pm 0.0074}$  \\
 & $s_{sub}$ &	0.4927$\pm$0.0067             &  0.8731$\pm$0.0073  \\
 & $m_{sub}$ &	0.4437$\pm$0.0034             &  1.0010$\pm$0.0080  \\
\hline
\end{tabular}
\caption{The cross comparison of average loss values (with standard error) using different loss functions during training and during testing. $l_{sub}$ is as in Equation~\eqref{eq:vocsubloss}. %As predicted by theory, 
Training with the same loss function as used during testing yields the best results.  Slack and margin rescaling fail due to the necessity of approximate inference, which results in a poor discriminant function.  The Lov\'{a}sz hinge trained on the appropriate loss yields the best performance in both cases.
}\label{tab:lossvoc}
\end{table}

\begin{table}[ht]\centering
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{2}{c|}{} & \multicolumn{2}{|c}{testing loss} \\
\cline{3-4}
\multicolumn{2}{c|}{} & $l_{sub}$ & 0-1  \\
\hline
\multirow{4}{*}{\rotatebox{90}{\small{training loss}}}
 & $l_{sub}$ &	$\mathbf{0.9447 \pm 0.0069}$  &  0.8786$\pm$0.0077  \\
 & 0-1       &	0.9877$\pm$0.0044             &  $\mathbf{0.8173 \pm 0.0061}$  \\
 & $s_{sub}$ &	0.9784$\pm$0.0052              &  0.8337$\pm$0.0054  \\
 & $m_{sub}$ &	0.9718$\pm$0.0041              &  0.9425$\pm$0.0054  \\
\hline
\end{tabular}
\caption{The cross comparison of average loss values (with standard error) using different loss functions during training and during testing. $l_{sub}$ is as in Equation~\eqref{eq:mixsubloss} (cf.\ comments for Table.~\ref{tab:lossvoc}).}\label{tab:lossvoc2}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%% figures of gap %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]\centering
\subfigure{\label{fig:gapTOY}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[ ]
{\includegraphics[width=0.45\linewidth]{gapVOC}}}
\subfigure{\label{fig:gapMIML}}\addtocounter{subfigure}{-2}
\subfigure{\subfigure[]
{\includegraphics[width=0.45\linewidth]{gapVOC2}}}
\caption{The primal-dual gap as a function of the number of cutting-plane iterations using the Lov\'{a}sz hinge with submodular loss, a SVM (labeled 0-1), and margin and slack rescaling with greedy inference (labeled $m_{sub}$ and $s_{sub}$). Fig.~\ref{fig:gapTOY} for the experiment using Equation~\eqref{eq:vocsubloss} and Fig.~\ref{fig:gapMIML} for Equation~\eqref{eq:mixsubloss}. This demonstrates that empirical convergence of the Lov\'{a}sz hinge is at a rate comparable to an SVM, and is feasible to optimize in practice for real-world problems.
}\label{fig:gap}
\end{figure}


==> SOSVMArXiv.tex <==
\section{Existing Convex Surrogates}\label{sec:SOSVM}

In this section, we analysis two existing convex surrogates namely margin rescaling and slack rescaling. We determine necessary and sufficient conditions for margin and slack rescaling to yield an extension of the underlying set loss function, and address their shortcoming in the complexity of subgradient computation.

%\section{Margin and Slack Rescaling}\label{sec:SOSVM}
A general problem is to learn a mapping $f$ from inputs $x\in\mathcal{X}$ to discrete outputs (labels) $y\in\mathcal{Y}$.  
The Structured Output SVM (SOSVM) is a popular framework for doing so in the regularized risk minimization framework~\cite{Taskar2003,tsochantaridis2005large}. The approach that SOSVM pursues is to learn a function $h:\mathcal{X}\times\mathcal{Y}\mapsto\mathbb{R}$ over input/output pairs from which a prediction can be derived by maximizing 
\begin{equation}
f(x) = \arg\max_{y} h(x,y)
\end{equation} 
over the response from a given input $x$. The SOSVM framework assumes $h$ to be represented by an inner product between an element of a reproducing kernel Hilbert space (RKHS) and some combined feature representation of inputs and outputs $\phi(x,y)$,
\begin{equation}\label{eq:SOSVMlinearCompatibilityFn}
h(x,y;w)=\langle w,\phi(x,y)\rangle
\end{equation}
although the notions of margin and slack rescaling may be applied to other function spaces, including random forests~\cite{Criminisi:2013:DFC:2462584} and deep networks~\cite{Bengio:2009:LDA:1658423.1658424}.

A bounded loss function $\Delta:\mathcal{Y\times Y}\to\mathbb{R}$ quantifies the loss associated with a prediction $\tilde{y}$ while the true value is $y$, and is used to re-scale the constraints. The margin-rescaling constraints and slack-rescaling constraints are:
\begin{align}%\label{eq:marginrescal}\centering
&\min_{w,\xi}  \frac{1}{2} \|w\|^2 + C \sum_{i=1}^{n} \xi_i,\quad \forall i,\forall \tilde{y}\in \mathcal{Y}: \label{eq:maxmargin}\\
&\langle w,\phi(x_i,y_i)\rangle
- \langle w,\phi(x_i,\tilde{y})\rangle \geq \Delta(y_i,\tilde{y})-\xi_i \label{eq:marginrescal}\\
&\text{or}\quad\langle w,\phi(x_i,y_i)\rangle
- \langle w,\phi(x_i,\tilde{y})\rangle \geq 1 - \frac{\xi_i}{\Delta(y_i,\tilde{y})} \label{eq:slackrescal}
\end{align}
respectively. A cutting plane algorithm is commonly used to solve it and one version of the approach with slack rescaling is shown in Algorithm~\ref{alg:cuttingplane}.
\begin{algorithm}[!t]
\caption{Cutting plane algorithm for solving the problem in Equation~\eqref{eq:maxmargin} and~\eqref{eq:slackrescal} -- Slack rescaling.}\label{alg:cuttingplane}
\begin{algorithmic}[1]
\STATE {Input: $(x_1,y_1),\cdots,(x_n,y_n),C,\epsilon$}
\STATE $S^i = \emptyset, \forall i = 1,\cdots,n$
\REPEAT 
\STATE for $i=1,\cdots,n$ do
\STATE $H(y_i) =  \Delta(y_i,\tilde{y}) ( 1 + h(x,\tilde{y}) - h(x,y_i))$
\STATE $\hat{y} = \arg\max_{\tilde{y}} H(y_i)$ \% most violated constraint %by permutation all possible $\tilde{y}$
\STATE $\xi^i = \max\{0,H(y_i)\}$
\IF {$H(\hat{y})>\xi^i+\epsilon$ }
\STATE $S^i:=S^i\cup \{y_i\}$
\STATE $w\leftarrow$ optimize Equation~\eqref{eq:maxmargin} with constraints defined by $\cup_i S^i$
\ENDIF
\UNTIL{no $S^i$ has changed during an iteration}
\RETURN $(w,\xi)$
\end{algorithmic}  
\end{algorithm}

In the sequel, we will consider the case that each $x_i \in \mathcal{X}$ is an ordered set of $p$ elements, and that $y_i \in \mathcal{Y}$ is a binary vector in $\{-1, +1\}^p$.  
We consider feature maps such that
\begin{equation}
\langle w, \phi(x,y) \rangle = \sum_{j=1}^p \langle w^j , x^j \rangle y^j .
\end{equation}
Given this family of joint feature maps, we may identify the $j$th dimension of $g$ (cf.\ Equation~\eqref{eq:binarySetPredictionSign}) with 
\begin{equation}\label{eq:g_func_x}
g^j(x) = \langle w^j, x^j \rangle.
\end{equation} 
Therefore $\arg\max_{y}h(x,y;w) = \operatorname{sign}(g(x))$ and 
\begin{equation}\label{eq:h_func_g}
h(x,y) = \langle g(x),y \rangle.
\end{equation} 
We emphasize that we may now drop the assumption that $g(x)$ be linearly parametrized by a vector $w$, and instead consider general (non-linear) functions.

\iffalse
We define
\begin{equation}
\phi(x_i,y_i) := \sum_{j=1}^p x_i^j \cdot y_i^j
\end{equation}
which is the specialization of the standard joint feature map for a random field model~\cite{Taskar2003,tsochantaridis2005large} to the case that there are no pairwise potentials.  In this way, the interdependency in the prediction process is introduced purely through the non-modularity of the loss function.
Given this choice of joint feature map, we have an equivalence between $\arg\max_y h(x,y;w)$, where $h$ is given in Equation~\eqref{eq:SOSVMlinearCompatibilityFn}, and $\operatorname{sign}(g(x))$ as specified in Equation~\eqref{eq:binarySetPredictionSign}.
\fi

%\subsection{Analysis of Margin and Slack Rescaling}\label{sec:AnalysisMSrescale}
\subsection{Extension}\label{sec:AnalysisMSrescale}

In order to analyse whether an operator $\mathbf{B}$ yields extensions of $\Delta$, we construct a mapping to a $p$-dimensional vector space using following definition:%s.t.\ $[v]_i = 1 - g(x^i,y^{*i})+g(x^i,y^i) = 1-\langle w, x^i \rangle y^i$, $i=\{1,\dots,p\}$ and we use the following definition:
\begin{defin}\label{def:extension}
A convex surrogate function $\mathbf{B} \Delta(y,\cdot)$ is an extension when $\mathbf{B} \Delta(y,\cdot) = \Delta(y,\cdot)$ on the vertices of the 0-1 unit cube under the mapping to $\mathbb{R}^p$ (cf.\ Fig.~\ref{fig:visualization}): % to a $p$-dimensional vector space s.t.
\begin{align}
j=&\{1,\dots,p\},\quad [u]^j = 1- g^j(x) y^j \label{eq:mapping2unitcube}
\end{align}
\end{defin}
%\mynewcorr{In practice, in the case that $y\in \{-1, +1\}^{p}$, we can translate the axe to $[u]^j = 1- g^j(x) (y^j-f(x)) $ in order to first have the vertices of the unit cube coinciding with $\Delta$.}

In the sequel, we will use the notation for $l : \mathcal{P}(V) \mapsto \mathbb{R}$ as in Equation~\eqref{eq:delta_l}.
%In the sequel, we define $l : \mathcal{P}(\{1,\dots,p\}) \mapsto %\mathbb{R})$ as 
%\begin{equation}
%l(\mathbf{I}) := \Delta(y,y\odot v)
%\end{equation}
%where $\odot$ is the Hadamard product and
%\begin{equation}
%[v]^i = \begin{cases} -1, & \text{ if } i \in \mathbf{I}\\
%+1, & \text{ otherwise}. \end{cases}
%\end{equation}
% $l := \Delta(y,\cdot)$ for brevity. 
 Note that at the vertices, %$\Delta$ have actually the values as following: 
$\Delta(y,\cdot)$ has the following values: 
\begin{align}
\label{eq:l_dot_empty}
&l(\emptyset)\ \textrm{at}\ \mathbf{0}_p\\
\label{eq:l_dot_gene}
&l(\mathbf{I})\ \textrm{at}\  \{v|v\in \{0,1\}^p,v_i=1\Leftrightarrow
 i\in \mathbf{I} \}
\end{align}
We call %the vertices (\ref{eq:l_dot_empty}) as \textit{the origin}, and 
\eqref{eq:l_dot_gene} the value of $l$ at \textit{the vertex $\mathbf{I}$}. 
%By Definition~\ref{def:extension}, at vertices $\mathbf{I}$ we have $[u]^i = 1 \iff \ g(x^i) =0$ for $i\in \mathbf{I}$ and $[u]^i = 0,\ g(x^i,y^{*i})-g(x^i,y^i) =1$ for $i\notin\mathbf{I}$.

% say something about the cutting plane, convex surrogates, extension

We denote the operators for margin and slack rescaling that map the loss function to its convex surrogates $\mathbf{M}$ and $\mathbf{S}$, respectively.  These operators have the same signature as $\mathbf{B}$ in Equation~\eqref{eq:ConvSurrogateOperatorSig}.
\begin{align}
\label{eq:upbound_m}
&\mathbf{M}\Delta(y,g(x)):=\max_{\tilde{y} \in \mathcal{Y}}\Delta(y,\tilde{y})+\langle g(x),\tilde{y} \rangle - \langle g(x),y \rangle\\
\label{eq:upbound_s}
&\mathbf{S}\Delta(y,g(x)):=\max_{\tilde{y} \in \mathcal{Y}}\Delta(y,\tilde{y})\big(1+ \langle g(x),\tilde{y} \rangle -\langle g(x),y \rangle \big)
\end{align}
respectively.

\subsection{Slack rescaling}
\begin{pro}\label{pro:SlackIncreasing}
$\mathbf{S}\Delta(y, \cdot)$ is an extension of a set function $\Delta(y,\cdot)$ iff $\Delta(y,\cdot)$ is an increasing function.
\end{pro}

\begin{proof}
First we demonstrate the necessity. Given $\mathbf{S}\Delta(y, \cdot)$ an extension of $\Delta(y,\cdot)$, we analyse whether $\Delta(y,\cdot)$ is an increasing function. Specifically, there are two cases to determine the values of $\mathbf{S}\Delta(y, \cdot)$:
\begin{enumerate}
\item if $u = \mathbf{0},\ \mathbf{S}\Delta(y, 
g(x)) = l(\varnothing)$ according to Equation~\eqref{eq:delta_l}, where $u$ is defined as in Equation~\eqref{eq:mapping2unitcube}.
\item if $u \in \mathbb{R}^p \setminus \{\mathbf{0}\}$, let $\mathbf{I}=\{i| u^{i}\neq 0\}$, then according to Equation~\eqref{eq:upbound_s}, $\mathbf{S}\Delta(y, g(x))$ takes the value of the following equation:
\begin{equation}
\label{eq:S_yneqy}
\max_{\mathbf{I} \in \mathcal{P}(V)}\ l(\mathbf{I})\big(1-
\sum_{i\in\mathbf{I}} g^i(x) y^{i}\big)
\end{equation}
\end{enumerate}
As $\mathbf{S}\Delta(y,g(x))$ is an extension of $\Delta(y,\operatorname{sign}(g(x)))$, by Definition~\ref{def:extension}, $\mathbf{S}\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertices as in (\ref{eq:l_dot_empty}) and (\ref{eq:l_dot_gene}). Note that it is trivial when $u=\mathbf{0}$ so the first case is always true for arbitrary (including increasing) $l$.  

Considering the second case when $\mathbf{S}\Delta(y,g(x))$ is equal to Equation~\eqref{eq:S_yneqy}, let $\mathbf{I}_2 = \arg\max_{\mathbf{I} \in \mathcal{P}(V)} l(\mathbf{I}) \big(1-\sum_{i\in\mathbf{I}} g^i(x) y^{i}\big)$. 
%To be more precise, we denote $\mathbf{I}_1$ the set of vertices that differ between $y$ and $\tilde{y}$ $\mathbf{S}\Delta(y, \cdot) =\max_y l( \mathbf{I}_1)[1-\sum_{i\in\mathbf{I}_1}\big( g(x^i,y^{*i})-g(x^i,y^i)\big)]$. 
%If it is supposed to yield with $\Delta(y,\cdot)$ at vertices $\mathbf{I}_2$, namely $[u]_i = 1,\ g(x^i,y^{*i})-g(x^i,y^i) =0$ for $i\in \mathbf{I}_2$ and $[u]_i = 0,\ g(x^i,y^{*i})-g(x^i,y^i) =1$ for $i\notin\mathbf{I}_2$, and $\mathbf{I}_1$ and $\mathbf{I}_2$ are not necessary the same. 
As $\mathbf{S}\Delta(y,g(x))$ is an extension, $\mathbf{S}\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertex $\mathbf{I}_2$. %Using the notation $\mathbf{N}:=\{1,\dots,p\}$ to denote the entire set of all indices, we get
\begin{align}
%\begin{split}
\label{eq:S_gene}
\!\!\!\!\!\forall\mathbf{I}_1 \in \mathcal{P}(V) \setminus \{ \emptyset \}, \ l( \mathbf{I}_2)\geq l( \mathbf{I}_1) \left(1 -|(V \setminus \mathbf{I}_2)\cap\mathbf{I}_1|\right)
%\end{split}
\end{align}
This leads also to two cases,
\begin{enumerate}
\item if $|(V \setminus \mathbf{I}_2)\cap\mathbf{I}_1|=0$, $(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1=\emptyset$, which implies $\mathbf{I}_1\subseteq\mathbf{I}_2$, 
then from Equation~\eqref{eq:S_gene} we get $l(\mathbf{I}_2) \geq l(\mathbf{I}_1)$. This implies that $l$ and therefore $\Delta$ are increasing;
\item if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|\geq 1$, this means the rhs of Equation~\eqref{eq:S_gene} is negative, then it turns out to be redundant with $l( \mathbf{I}_2)\geq 0$ which is always true.
\end{enumerate}
To conclude, given $\mathbf{S}\Delta(y, \cdot)$ is an extension of a set function $\Delta(y,\cdot)$, it is always the case that $\Delta$ is increasing.

To demonstrate the sufficiency, we need to show Equation~\eqref{eq:S_gene} is always true if $l$ is increasing. We note that \eqref{eq:S_gene} holds if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|=0$, because if $\mathbf{I}_1\subseteq\mathbf{I}_2$ then  $l(\mathbf{I}_2) \geq l(\mathbf{I}_1)$. Then if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|\geq 1$, \eqref{eq:S_gene} always holds even for arbitrary $l$. We conclude that $\mathbf{S}\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertices when Equation~\eqref{eq:l_dot_gene} holds. As for the case of Equation~\eqref{eq:l_dot_empty}, it is trivial as $u=\mathbf{0}$. So $\mathbf{S}\Delta(y,\cdot)$ yields a extension of $\Delta(y,\cdot)$ if $\Delta(y,\cdot)$ is increasing.
\end{proof}

\subsection{Margin rescaling}
It is a necessary, but not sufficient condition that $\Delta(y,\tilde{y})$ be increasing for margin rescaling to yield an extension.  However, we note that for all increasing $\Delta(y,\tilde{y})$ there exists a positive scaling $\gamma \in \mathbb{R}$ such that margin rescaling yields an extension.  This is an important result for regularized risk minimization as we may simply rescale $\Delta$ to guarantee that margin rescaling yields an extension, and simultaneously scale the regularization parameter such that the relative contribution of the regularizer and loss is unchanged at the vertices of the unit cube. 
%In the sequel, we denote $l := \Delta(y,\cdot)$ for brevity.

\begin{pro}\label{pro:gamma_exist}
% same here, should we say \Delta is inreasing or l is increasing
For all increasing set functions $l$ such that $\exists y$ for which $\mathbf{M}\Delta(y, \cdot)$ is not an extension of $\Delta(y,\cdot)$,
% i.e $\exists \widetilde{\mathbf{y}}$, $\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}}) \neq \mathbf{M}\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}})$, then 
we can always find a positive scale factor $\gamma$ specific to $l$ such that margin rescaling yields an extension. We denote $\mathbf{M} \gamma\Delta$ and $\gamma\Delta$ as the rescaled functions. %that can make $\gamma\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}}) = \mathbf{M}\gamma\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}})$.
\end{pro}

\begin{proof}
Similar to Proposition~\ref{pro:SlackIncreasing}, we analyse two cases to determine the values of $\mathbf{M}\gamma\Delta(y,g(x))$:
\begin{enumerate}
\item if $u=\mathbf{0},\ \mathbf{M}\gamma\Delta(y,g(x)) = \gamma l(\varnothing)$ where $u$ is defined as in Equation~\eqref{eq:mapping2unitcube}. It is typically the case that $l(\varnothing)=0$, but this is not a technical requirement.
\item if $u\neq \mathbf{0}$, let $\mathbf{I}=\{i| u^i\neq 0\}$, then $\mathbf{M}\gamma\Delta(y,g(x))$ takes the value of the following equation:
\begin{equation}
\label{eq:yneqy}
\max_{\mathbf{I}\in \mathcal{P}(V)}\  \gamma l(\mathbf{I})-
\sum_{i\in\mathbf{I}} g^i(x) y^{i}  
\end{equation}
\end{enumerate}
%With the \textbf{Proposition \ref{pro:gamma_exist}} taken into account, take (\ref{eq:l_dot_empty}) into Eq.\ref{eq:xi}, the scale factor should satisfied:
To satisfy Definition~\ref{def:extension}, we must find a $\gamma > 0$ such that $\mathbf{M}\gamma\Delta(y,g(x)) = \gamma\Delta(y,\operatorname{sign}(g(x)))$ at the vertices. Note that it is trivial when $u=\mathbf{0}$ so the first case is true for arbitrary $\gamma > 0$.  

For the second case as in Equation~\eqref{eq:yneqy}, 
%Then combining the Eq.\ref{eq:l_dot_gene} and Eq.\ref{eq:xi} while being scaled, 
%In the case with (\ref{eq:l_dot_gene}) (the non-original value of $\Delta$), 
let $\mathbf{I}_2 = \arg\max_{\mathbf{I} \in \mathcal{P}(V)}\big( l(\mathbf{I})-\sum_{i\in\mathbf{I}} g^i(x) y^{i}\big)$. 
We have $\mathbf{M}\gamma\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertices $\mathbf{I}_2$ according to the extension. The scale factor should satisfy:
\begin{equation}
%\begin{split}
\label{eq:gamma_gene}
\!\!\!\forall\mathbf{I}_1 \in \mathcal{P}(V) \setminus \{ \emptyset \}, \ \gamma\big(l( \mathbf{I}_2)-l( \mathbf{I}_1) \big) \geq -|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|
%\end{split}
\end{equation}
which leads to the following cases:
\begin{enumerate}
\item if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|=0$, we have $(V \setminus \mathbf{I}_2)\cap\mathbf{I}_1=\emptyset$, which implies $\mathbf{I}_1\subseteq\mathbf{I}_2$. Equation~\eqref{eq:gamma_gene} reduces to 
\begin{equation}
\label{eq:gamma_gene_1}
\gamma\big(l(\mathbf{I}_2)-l(\mathbf{I}_1) \big)\geq 0
\end{equation}
and $l$ is an increasing function so $l( \mathbf{I}_1)\leq l(\mathbf{I}_2) $ and Equation~\eqref{eq:gamma_gene_1} is always true as $\gamma>0$.
\item if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|\neq0$, we need to discuss the relationship between $l( \mathbf{I}_1)$ and $l( \mathbf{I}_2)$:
\begin{enumerate}
\item if $l( \mathbf{I}_2)=l( \mathbf{I}_1)$, then  Equation~\eqref{eq:gamma_gene_1} becomes $0\geq-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|$, for which the rhs is negative so it is always true.
\item if $l( \mathbf{I}_2)>l( \mathbf{I}_1)$, then
\begin{equation}
\label{eq:gamma_gene_2.1}
\gamma\geq\frac{-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|}{l( \mathbf{I}_2)-l( \mathbf{I}_1)}
\end{equation}
for which the rhs is negative so it is redundant with $\gamma>0$ .
\item if $l(\mathbf{I}_2)<l(\mathbf{I}_1)$, then
\begin{equation}
\label{eq:gamma_gene_2.2}
\gamma\leq\frac{-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|}{l( \mathbf{I}_2)-l( \mathbf{I}_1)}
\end{equation}
for which the rhs is \emph{strictly} positive so it becomes an upper bound on $\gamma$ .
\end{enumerate}
\end{enumerate}
In summary the scale factor $\gamma$ should satisfy the following constraint for an increasing loss function $l$: %, which in the meantime prove the existence, on the only condition that $l$ should be an increasing function.
\begin{align*}
\forall\mathbf{I}_1,\mathbf{I}_2 \in \mathcal{P}(V) \setminus \{ \emptyset \}, 
%,&\mathbf{I}_1\neq\emptyset,\mathbf{I}_2\neq\emptyset,\  \\ &
0<\gamma\leq \frac{-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|}{l(\mathbf{I}_2)-l(\mathbf{I}_1)} 
\end{align*}
Finally, we note that the rightmost ratio is always strictly positive.
\end{proof}

\subsection{Complexity of subgradient computation}

Although we have proven that slack and margin rescaling yield extensions to the underlying discrete loss under fairly general conditions, %\mycorr{which is actually not a prevalent analysis perspective in the existing literature}, 
their key shortcoming is in the complexity of the computation of subgradients for submodular losses.  The subgradient computation for slack and margin rescaling requires the computation of 
\begin{equation}
\arg\max_{\tilde{y}} \Delta(y,\tilde{y}) ( 1 + h(x,\tilde{y}) - h(x,y))
\end{equation}
and 
\begin{equation}
\arg\max_{\tilde{y}} \Delta(y,\tilde{y}) + h(x,\tilde{y}), 
\end{equation}
respectively.  Both of these functions require the maximization of the loss, which corresponds to supermodular minimization in the case of a submodular loss.  This computation is NP-hard, and such loss functions are not feasible with these existing methods in practice.  Furthermore, approximate inference, e.g.\ based on~\cite{Nemhauser1978}, leads to poor convergence when used to train a structured output SVM resulting in a high error rate~\cite{Finley:2008}.  We therefore introduce the Lov\'{a}sz hinge as an alternative operator to construct feasible convex surrogates for submodular losses.


==> SOSVM_new.tex <==

\section{Existing Convex Surrogates}\label{sec:SOSVM}
%\section{Margin and Slack Rescaling}\label{sec:SOSVM}

A general problem is to learn a mapping $f$ from inputs $x\in\mathcal{X}$ to discrete outputs (labels) $y\in\mathcal{Y}$.  
The Structured Output SVM (SOSVM) is a popular framework for doing so in the regularized risk minimization framework. The approach that SOSVM pursues is to learn a function $h:\mathcal{X}\times\mathcal{Y}\mapsto\mathbb{R}$ over input/output pairs from which a prediction can be derived by maximizing $f(x) = \arg\max_{y} h(x,y)$ over the response from a given input $x$. The SOSVM framework assumes $h$ to be represented by an inner product between an element of a reproducing kernel Hilbert space (RKHS) and some combined feature representation of inputs and outputs $\phi(x,y)$,
\begin{equation}\label{eq:SOSVMlinearCompatibilityFn}
h(x,y;w)=\langle w,\phi(x,y)\rangle
\end{equation}
although the notions of margin and slack rescaling may be applied to other function spaces, including random forests and deep networks.

A bounded loss function $\Delta:\mathcal{Y\times Y}\to\mathbb{R}$ quantifies the loss associated with a prediction $\tilde{y}$ while the true value is $y$, and is used to re-scale the constraints. The margin-rescaling constraints and slack-rescaling constraints are:
\begin{align}%\label{eq:marginrescal}\centering
&\min_{w,\xi}  \frac{1}{2} \|w\|^2 + C \sum_{i=1}^{n} \xi_i,\quad \forall i,\forall \tilde{y}\in \mathcal{Y}: \\
&\langle w,\phi(x_i,y_i)\rangle
- \langle w,\phi(x_i,\tilde{y})\rangle \geq \Delta(y_i,\tilde{y})-\xi_i\\
&\text{or}\quad\langle w,\phi(x_i,y_i)\rangle
- \langle w,\phi(x_i,\tilde{y})\rangle \geq 1 - \frac{\xi_i}{\Delta(y_i,\tilde{y})}
\end{align}
respectively.

In the sequel, we will consider the case that each $x_i \in \mathcal{X}$ is an ordered set of $p$ elements in a RKHS, $\mathcal{H}$, and that $y_i \in \mathcal{Y}$ is a binary vector in $\{-1, +1\}^p$.  
We consider feature maps such that
\begin{equation}
\langle w, \phi(x_i,y_i) \rangle = \sum_{j=1}^p \langle w^j , x_i^j \rangle y_i^j .
\end{equation}
Given this family of joint feature maps, we may identify the $j$th dimension of $g$ (cf.\ Equation~\eqref{eq:binarySetPredictionSign}) with $\langle w^j, x_i^j \rangle$.  Therefore $\arg\max_{y}h(x,y;w) = \operatorname{sign}(g(x))$ and $h(x,y) = \langle g(x),y \rangle$.

\iffalse
We define
\begin{equation}
\phi(x_i,y_i) := \sum_{j=1}^p x_i^j \cdot y_i^j
\end{equation}
which is the specialization of the standard joint feature map for a random field model~\cite{Taskar2003,tsochantaridis2005large} to the case that there are no pairwise potentials.  In this way, the interdependency in the prediction process is introduced purely through the non-modularity of the loss function.
Given this choice of joint feature map, we have an equivalence between $\arg\max_y h(x,y;w)$, where $h$ is given in Equation~\eqref{eq:SOSVMlinearCompatibilityFn}, and $\operatorname{sign}(g(x))$ as specified in Equation~\eqref{eq:binarySetPredictionSign}.
\fi

\subsection{Analysis of Margin and Slack Rescaling}\label{sec:AnalysisMSrescale}

We now turn to the problem of determining necessary and sufficient conditions for margin and slack rescaling to yield an extension of the underlying set loss function.
We denote the operators for margin and slack rescaling that map the loss function to its convex surrogate $\mathbf{M}$ and $\mathbf{S}$, respectively.  These operators have the same signature as $\mathbf{B}$ in Equation~\eqref{eq:ConvSurrogateOperatorSig}.
\iffalse
We are now interested in the general(??) problem of learning functions $f:\mathcal{X}\to\mathcal{\overline{Y}}$ between input spaces $\mathcal{X}$ and the extended continuous output space $\mathcal{\overline{Y}} := \mathbb{R}^p$, accompanied with a function $t$ mapping this extended space to the original output space $\mathcal{Y}$. A binary classification problem with $p$ $d$-dimensional patterns is taken into consideration as following, with $\mathcal{X}:=\mathbb{R}^{d\times p}$ as the input space and $\mathcal{Y}:=(y^1,\dots,y^p)\in \{-1,+1\}^p$ the output space. To find the final prediction, we will threshold the real-valued output $f:=\textrm{sign}(g)$.%$t(f):=\textrm{sign}(f)$.
%\begin{displaymath}
%\mathcal{X}:=\mathbb{R}^{d\times n}\qquad
%\mathcal{Y}:=(\mathbf{y}_1,\cdots,\mathbf{y}_n)\in \{-1,+1\}^n
%\end{displaymath}

The goal is to find a function composition $t\cdot f$ such that the risk $\mathcal{R}^{\Delta}(f)$ (cf.\ Equation~\eqref{eq:Risk}) is minimized. 
The approach we pursue is to learn a function $g:\mathcal{X}\times\mathcal{F}\to\mathbb{R}$ over input-output pairs from which we can derive a prediction by maximizing $g$ :
\begin{equation*}
t(f(\mathbf{x})):=\arg\max_\mathbf{y} g(\mathbf{x},\mathbf{y})
\end{equation*}
Instead of assuming $g$ to be linear in some combined feature representation of inputs and outputs~\cite{tsochantaridis2005large}, we maintain for now this general form.
As the loss function $\Delta$ maps from $\mathcal{Y}\times\mathcal{Y}$ to $\mathbb{R}$, we denote margin and slack rescaling as two operators, $\mathbf{M}$ and $\mathbf{S}$, which map the function $\Delta$ on the discrete space to functions $\mathbf{M}\Delta$  and $\mathbf{S}\Delta$ on a continuous space .
\begin{align*}
\mathbf{M}:\big(\mathcal{Y}\times\mathcal{Y}\to\mathbb{R}\big)
&\to\big(\mathcal{Y}\times\mathcal{\overline{Y}}\to\mathbb{R}\big)
\equiv
\big(\mathcal{Y}\times\mathcal{Y}\to\mathbb{R}\big)
&\to\big(\mathcal{Y}\times(\mathcal{Y}\to\mathbb{R})\to\mathbb{R}\big)\\
\mathbf{S}:\big(\mathcal{Y}\times\mathcal{Y}\to\mathbb{R}\big)
&\to\big(\mathcal{Y}\times\mathcal{\overline{Y}}\to\mathbb{R}\big)
\equiv
\big(\mathcal{Y}\times\mathcal{Y}\to\mathbb{R}\big)
&\to\big(\mathcal{Y}\times(\mathcal{Y}\to\mathbb{R})\to\mathbb{R}\big)
\end{align*} 
which specifically are expressed as following: 
\fi
\begin{align}
\label{eq:upbound_m}
&\mathbf{M}\Delta(y,g(x)):=\max_{\tilde{y} \in \mathcal{Y}}\Delta(y,\tilde{y})+\langle g(x),\tilde{y} \rangle - \langle g(x),y \rangle\\
\label{eq:upbound_s}
&\mathbf{S}\Delta(y,g(x)):=\max_{\tilde{y} \in \mathcal{Y}}\Delta(y,\tilde{y})\big(1+ \langle g(x),\tilde{y} \rangle -\langle g(x),y \rangle \big)
\end{align}
respectively.

In order to analyse whether $\mathbf{M}\Delta$ and $\mathbf{S}\Delta$ are extensions of $\Delta$, we construct a mapping to a $p$-dimensional vector space using following definition:%s.t.\ $[v]_i = 1 - g(x^i,y^{*i})+g(x^i,y^i) = 1-\langle w, x^i \rangle y^i$, $i=\{1,\dots,p\}$ and we use the following definition:
\iffalse
\begin{defin}\label{def:ext}
A convex surrogate function $\mathbf{B} \Delta(y^{*},\cdot)$ is an extension when $\mathbf{B} \Delta(y,\cdot) = \Delta(y,\cdot)$ on the vertices of the 0-1 unit cube under this mapping. (Figure~\ref{fig:m+-}).
\end{defin}
\fi
\begin{defin}\label{def:extention}
A convex surrogate function $\mathbf{B} \Delta(y,\cdot)$ is an extension when $\mathbf{B} \Delta(y,\cdot) = \Delta(y,\cdot)$ on the vertices of the 0-1 unit cube under the mapping to $\mathbb{R}^p$ (cf.\ Fig.~\ref{fig:visualization}): % to a $p$-dimensional vector space s.t.
\begin{align}
i=&\{1,\dots,p\},\quad [u]^i = 1-\langle w, x^i \rangle y^i \label{eq:mapping2unitcube}
\end{align}
\end{defin}
In the sequel, we will use the notation for $l : \mathcal{P}(V) \mapsto \mathbb{R}$ as in Equation~\eqref{eq:delta_l}.
%In the sequel, we define $l : \mathcal{P}(\{1,\dots,p\}) \mapsto %\mathbb{R})$ as 
%\begin{equation}
%l(\mathbf{I}) := \Delta(y,y\odot v)
%\end{equation}
%where $\odot$ is the Hadamard product and
%\begin{equation}
%[v]^i = \begin{cases} -1, & \text{ if } i \in \mathbf{I}\\
%+1, & \text{ otherwise}. \end{cases}
%\end{equation}
% $l := \Delta(y,\cdot)$ for brevity. 
 Note that at the vertices, %$\Delta$ have actually the values as following: 
$\Delta(y,\cdot)$ has the following values: 
\begin{align}
\label{eq:l_dot_empty}
&l(\varnothing)\ \textrm{at}\ \mathbf{0}_p\\
\label{eq:l_dot_gene}
&l(\mathbf{I})\ \textrm{at}\  \{v|v\in \{0,1\},v_i=1\Leftrightarrow
 i\in \mathbf{I} \}
\end{align}
\iffalse
\begin{align}
\label{eq:l_dot_empty}
&l(\varnothing)\ \textrm{at}\ [\underbrace{0,\cdots,0}_{p}]\\
\label{eq:l_dot_gene}
&l(\mathbf{I})\ \textrm{at}\ \sum_{i\in\mathbf{I}}[\underbrace{0,\cdots,1,\cdots,0}_{1\ \textrm{at}\ i^{th}}]
\end{align}
\fi 
We call %the vertices (\ref{eq:l_dot_empty}) as \textit{the origin}, and 
\eqref{eq:l_dot_gene} the value of $l$ at \textit{the vertex $\mathbf{I}$}. 
%By Definition~\ref{def:extention}, at vertices $\mathbf{I}$ we have $[u]^i = 1 \iff \ g(x^i) =0$ for $i\in \mathbf{I}$ and $[u]^i = 0,\ g(x^i,y^{*i})-g(x^i,y^i) =1$ for $i\notin\mathbf{I}$.

\subsection{Slack rescaling}
\begin{pro}\label{pro:SlackIncreasing}
$\mathbf{S}\Delta(y, \cdot)$ is an extension of a set function $\Delta(y,\cdot)$ iff $\Delta(y,\cdot)$ is an increasing function.
\end{pro}
% should we say : \Delta is inreacing or l is increasing?????
\iffalse
\textit{Proof sketch.} We note that slack rescaling yields a piecewise linear surrogate function, with one linear component per element of the output space.  The equality of the extension and the discrete function at a given vertex of the unit cube is achieved when the piecewise linear component associated with that vertex has a higher value at the vertex than all other piecewise linear components.  This system of inequalities directly leads to constraints that $\Delta(y,\cdot)$ be increasing. \qed
\fi
\begin{proof}
First we demonstrate the necessity. Given $\mathbf{S}\Delta(y, \cdot)$ an extension of $\Delta(y,\cdot)$, we analyse whether $\Delta(y,\cdot)$ is an increasing function. Specifically, there are two cases to determine the values of $\mathbf{S}\Delta(y, \cdot)$:
\begin{enumerate}
\item if $u = \mathbf{0},\ \mathbf{S}\Delta(y, 
g(x)) = l(\varnothing)$ according to Equation~\eqref{eq:delta_l}, where $u$ is defined as in Equation~\eqref{eq:mapping2unitcube}.
\item if $u \in \mathbb{R}^p \setminus \{\mathbf{0}\}$, let $\mathbf{I}=\{i| u^{i}\neq 0\}$, then according to Equation~\eqref{eq:upbound_s}, $\mathbf{S}\Delta(y, g(x))$ takes the value of the following equation:
\begin{equation}
\label{eq:S_yneqy}
\max_{\mathbf{I} \in \mathcal{P}(V)}\ l(\mathbf{I})\big(1-
\sum_{i\in\mathbf{I}} \langle w, x^i \rangle y^{i}\big)
\end{equation}
\end{enumerate}
As $\mathbf{S}\Delta(y,g(x))$ is an extension of $\Delta(y,\operatorname{sign}(g(x)))$, by Definition~\ref{def:extention}, $\mathbf{S}\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertices as in (\ref{eq:l_dot_empty}) and (\ref{eq:l_dot_gene}). Note that it is trivial when $u=\mathbf{0}$ so the first case is always true for arbitrary (including increasing) $l$.  

Considering the second case when $\mathbf{S}\Delta(y,g(x))$ is equal to Equation~\eqref{eq:S_yneqy}, let $\mathbf{I}_2 = \arg\max_{\mathbf{I} \in \mathcal{P}(V)} l(\mathbf{I}) \big(1-\sum_{i\in\mathbf{I}}\langle w, x^i \rangle y^{i}\big)$. 
%To be more precise, we denote $\mathbf{I}_1$ the set of vertices that differ between $y$ and $\tilde{y}$ $\mathbf{S}\Delta(y, \cdot) =\max_y l( \mathbf{I}_1)[1-\sum_{i\in\mathbf{I}_1}\big( g(x^i,y^{*i})-g(x^i,y^i)\big)]$. 
%If it is supposed to yield with $\Delta(y,\cdot)$ at vertices $\mathbf{I}_2$, namely $[u]_i = 1,\ g(x^i,y^{*i})-g(x^i,y^i) =0$ for $i\in \mathbf{I}_2$ and $[u]_i = 0,\ g(x^i,y^{*i})-g(x^i,y^i) =1$ for $i\notin\mathbf{I}_2$, and $\mathbf{I}_1$ and $\mathbf{I}_2$ are not necessary the same. 
As $\mathbf{S}\Delta(y,g(x))$ is an extension, $\mathbf{S}\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertex $\mathbf{I}_2$. %Using the notation $\mathbf{N}:=\{1,\dots,p\}$ to denote the entire set of all indices, we get
\begin{align}
%\begin{split}
\label{eq:S_gene}
\!\!\!\!\!\forall\mathbf{I}_1 \in \mathcal{P}(V) \setminus \{ \emptyset \}, \ l( \mathbf{I}_2)\geq l( \mathbf{I}_1) \left(1 -|(V \setminus \mathbf{I}_2)\cap\mathbf{I}_1|\right)
%\end{split}
\end{align}
This leads also to two cases,
\begin{enumerate}
\item if $|(V \setminus \mathbf{I}_2)\cap\mathbf{I}_1|=0$, $(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1=\emptyset$, which implies $\mathbf{I}_1\subseteq\mathbf{I}_2$, 
then from Equation~\eqref{eq:S_gene} we get $l(\mathbf{I}_2) \geq l(\mathbf{I}_1)$. This implies that $l$ and therefore $\Delta$ are increasing;
\item if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|\geq 1$, this means the rhs of Equation~\eqref{eq:S_gene} is negative, then it turns out to be redundant with $l( \mathbf{I}_2)\geq 0$ which is always true.
\end{enumerate}
To conclude, given $\mathbf{S}\Delta(y, \cdot)$ is an extension of a set function $\Delta(y,\cdot)$, it is always the case that $\Delta$ is increasing.

To demonstrate the sufficiency, we need to show Equation~\eqref{eq:S_gene} is always true if $l$ is increasing. We note that \eqref{eq:S_gene} holds if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|=0$, because if $\mathbf{I}_1\subseteq\mathbf{I}_2$ then  $l(\mathbf{I}_2) \geq l(\mathbf{I}_1)$. Then if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|\geq 1$, \eqref{eq:S_gene} always holds even for arbitrary $l$. We conclude that $\mathbf{S}\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertices when Equation~\eqref{eq:l_dot_gene} holds. As for the case of Equation~\eqref{eq:l_dot_empty}, it is trivial as $u=\mathbf{0}$. So $\mathbf{S}\Delta(y,\cdot)$ yields a extension of $\Delta(y,\cdot)$ if $\Delta(y,\cdot)$ is increasing.
\end{proof}

\subsection{Margin rescaling}
It is a necessary, but not sufficient condition that $\Delta(y,\tilde{y})$ be increasing for margin rescaling to yield an extension.  However, we note that for all increasing $\Delta(y,\tilde{y})$ there exists a positive scaling $\gamma \in \mathbb{R}$ such that margin rescaling yields an extension.  This is an important result for regularized risk minimization as we may simply rescale $\Delta$ to guarantee that margin rescaling yields an extension, and simultaneously scale the regularization parameter such that the relative contribution of the regularizer and loss is unchanged at the vertices of the unit cube. 
%In the sequel, we denote $l := \Delta(y,\cdot)$ for brevity.

\begin{pro}\label{pro:gamma_exist}
% same here, should we say \Delta is inreasing or l is increasing
For all increasing set functions $l$ such that $\exists y$ for which $\mathbf{M}\Delta(y, \cdot)$ is not an extension of $\Delta(y,\cdot)$,
% i.e $\exists \widetilde{\mathbf{y}}$, $\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}}) \neq \mathbf{M}\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}})$, then 
we can always find a positive scale factor $\gamma$ specific to $l$ such that margin rescaling yields an extension. We denote $\mathbf{M} \gamma\Delta$ and $\gamma\Delta$ as the rescaled functions. %that can make $\gamma\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}}) = \mathbf{M}\gamma\Delta(\mathbf{y}^*,\widetilde{\mathbf{y}})$.
\end{pro}

\begin{proof}
Similar to Proposition~\ref{pro:SlackIncreasing}, we analyse two cases to determine the values of $\mathbf{M}\gamma\Delta(y,g(x))$:
\begin{enumerate}
\item if $u=\mathbf{0},\ \mathbf{M}\gamma\Delta(y,g(x)) = \gamma l(\varnothing)$ where $u$ is defined as in Equation~\eqref{eq:mapping2unitcube}. It is typically the case that $l(\varnothing)=0$, but this is not a technical requirement.
\item if $u\neq \mathbf{0}$, let $\mathbf{I}=\{i| u^i\neq 0\}$, then $\mathbf{M}\gamma\Delta(y,g(x))$ takes the value of the following equation:
\begin{equation}
\label{eq:yneqy}
\max_{\mathbf{I}\in \mathcal{P}(V)}\  \gamma l(\mathbf{I})-
\sum_{i\in\mathbf{I}} \langle w, x^i \rangle y^{i}  
\end{equation}
\end{enumerate}
%With the \textbf{Proposition \ref{pro:gamma_exist}} taken into account, take (\ref{eq:l_dot_empty}) into Eq.\ref{eq:xi}, the scale factor should satisfied:
To satisfy Definition~\ref{def:extention}, we must find a $\gamma > 0$ such that $\mathbf{M}\gamma\Delta(y,g(x)) = \gamma\Delta(y,\operatorname{sign}(g(x)))$ at the vertices. Note that it is trivial when $u=\mathbf{0}$ so the first case is true for arbitrary $\gamma > 0$.  

For the second case as in Equation~\eqref{eq:yneqy}, 
%Then combining the Eq.\ref{eq:l_dot_gene} and Eq.\ref{eq:xi} while being scaled, 
%In the case with (\ref{eq:l_dot_gene}) (the non-original value of $\Delta$), 
let $\mathbf{I}_2 = \arg\max_{\mathbf{I} \in \mathcal{P}(V)}\big( l(\mathbf{I})-\sum_{i\in\mathbf{I}}\langle w, x^i \rangle y^{i}\big)$. 
We have $\mathbf{M}\gamma\Delta(y,g(x)) = \Delta(y,\operatorname{sign}(g(x)))$ at the vertices $\mathbf{I}_2$ according to the extension. The scale factor should satisfy:
\begin{equation}
%\begin{split}
\label{eq:gamma_gene}
\!\!\!\forall\mathbf{I}_1 \in \mathcal{P}(V) \setminus \{ \emptyset \}, \ \gamma\big(l( \mathbf{I}_2)-l( \mathbf{I}_1) \big) \geq -|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|
%\end{split}
\end{equation}
which leads to the following cases:
\begin{enumerate}
\item if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|=0$, we have $(V \setminus \mathbf{I}_2)\cap\mathbf{I}_1=\emptyset$, which implies $\mathbf{I}_1\subseteq\mathbf{I}_2$. Equation~\eqref{eq:gamma_gene} reduces to 
\begin{equation}
\label{eq:gamma_gene_1}
\gamma\big(l(\mathbf{I}_2)-l(\mathbf{I}_1) \big)\geq 0
\end{equation}
and $l$ is an increasing function so $l( \mathbf{I}_1)\leq l(\mathbf{I}_2) $ and Equation~\eqref{eq:gamma_gene_1} is always true as $\gamma>0$.
\item if $|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|\neq0$, we need to discuss the relationship between $l( \mathbf{I}_1)$ and $l( \mathbf{I}_2)$:
\begin{enumerate}
\item if $l( \mathbf{I}_2)=l( \mathbf{I}_1)$, then  Equation~\eqref{eq:gamma_gene_1} becomes $0\geq-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|$, for which the rhs is negative so it is always true.
\item if $l( \mathbf{I}_2)>l( \mathbf{I}_1)$, then
\begin{equation}
\label{eq:gamma_gene_2.1}
\gamma\geq\frac{-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|}{l( \mathbf{I}_2)-l( \mathbf{I}_1)}
\end{equation}
for which the rhs is negative so it is redundant with $\gamma>0$ .
\item if $l(\mathbf{I}_2)<l(\mathbf{I}_1)$, then
\begin{equation}
\label{eq:gamma_gene_2.2}
\gamma\leq\frac{-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|}{l( \mathbf{I}_2)-l( \mathbf{I}_1)}
\end{equation}
for which the rhs is \emph{strictly} positive so it becomes an upper bound on $\gamma$ .
\end{enumerate}
\end{enumerate}
In summary the scale factor $\gamma$ should satisfy the following constraint for an increasing loss function $l$: %, which in the meantime prove the existence, on the only condition that $l$ should be an increasing function.
\begin{align*}
\forall\mathbf{I}_1,\mathbf{I}_2 \in \mathcal{P}(V) \setminus \{ \emptyset \}, 
%,&\mathbf{I}_1\neq\emptyset,\mathbf{I}_2\neq\emptyset,\  \\ &
0<\gamma\leq \frac{-|(V\setminus \mathbf{I}_2)\cap\mathbf{I}_1|}{l(\mathbf{I}_2)-l(\mathbf{I}_1)} 
\end{align*}
Finally, we note that the rightmost ratio is always strictly positive.
\end{proof}

\subsection{Complexity of subgradient computation}

Although we have proven that slack and margin rescaling yield extensions to the underlying discrete loss under fairly general conditions, %\mycorr{which is actually not a prevalent analysis perspective in the existing literature}, 
their key shortcoming is in the complexity of the computation of subgradients for submodular losses.  The subgradient computation for slack and margin rescaling requires the computation of 
%\begin{equation}
$\arg\max_{\tilde{y}} \Delta(y,\tilde{y}) ( 1 + h(x,\tilde{y}) - h(x,y))$ 
%\end{equation}
and 
%\begin{equation}
$\arg\max_{\tilde{y}} \Delta(y,\tilde{y}) + h(x,\tilde{y})$, 
%\end{equation}
respectively.  Both of these functions require the maximization of the loss, which corresponds to supermodular minimization in the case of a submodular loss.  This computation is NP-hard, and such loss functions are not feasible with these existing methods in practice.  Furthermore, approximate inference, e.g.\ based on~\cite{Nemhauser1978}, leads to poor convergence when used to train a structured output SVM resulting in a high error rate~\cite{Finley:2008}.  We therefore introduce the Lov\'{a}sz hinge as an alternative operator to construct feasible convex surrogates for submodular losses.

==> SubmodularArXiv.tex <==

\section{Submodular Loss Functions}\label{sec:Submodular}
%\subsection{ERM problem}
In empirical risk minimization (ERM), we approximate the risk, $\mathcal{R}$ of a prediction function $f : \mathcal{X} \mapsto \mathcal{Y}$ by an empirical sum over losses incurred on a finite sample, using e.g.\ an i.i.d.\ sampling assumption~\cite{Vapnik:1995}:
\begin{equation}\label{eq:Risk}
%\begin{split}
%\mathcal{R}(f) &:= \int_{\mathcal{X} \times \mathcal{Y}} \Delta(y,f(x)) dP(x,y)\\ \underbrace{\approx}_{\text{i.i.d.}} 
\hat{\mathcal{R}}(f) := \frac{1}{n} \sum_{i=1}^{n} \Delta(y_i,f(x_i))
%\end{split}
\end{equation}
Central to the practical application of the ERM principle, one must approximate, or upper bound the discrete loss function $\Delta$ with a convex surrogate.  We will identify the creation of a convex surrogate for a specific loss function with an operator that maps a function with a discrete domain to one with a continuous domain.  In particular, we will study the case that the discrete domain is a set of $p$ binary predictions.  In this case we denote
\begin{align}
\mathcal{Y} &= \{-1, +1\}^{p}\\
f(x) &= \operatorname{sign}(g(x)) \label{eq:binarySetPredictionSign}\\
\Delta &: \{-1, +1 \}^{p} \times \{-1, +1 \}^{p} \mapsto \mathbb{R}_{+}\\
\mathbf{B} \Delta &: \{-1 , +1 \}^p \times \mathbb{R}^{p} \mapsto \mathbb{R} \label{eq:ConvSurrogateOperatorSig}
\end{align}
where $\mathbf{B}$ is an operator that constructs the surrogate loss function from $\Delta$, and $g : \mathcal{X} \mapsto \mathbb{R}^{p}$ is a parametrized prediction function to be optimized by ERM.

A key property is the relationship between $\mathbf{B} \Delta$ and $\Delta$.  In particular, we are interested in when a given surrogate strategy $\mathbf{B}\Delta$ yields an \emph{extension} of $\Delta$ (cf.\ Definition~\ref{def:extension}).  We make this notion formal by identifying $\{-1, +1\}^{p}$ with a given $p$-dimensional unit hypercube of $\mathbb{R}^p$ .  We say that $\mathbf{B} \Delta(y, \cdot)$ is an extension of $\Delta(y,\cdot)$ iff the functions are equal over the vertices of this unit hypercube.  We focus on function extensions as 
they ensure a tight relationship between the discrete loss and the convex surrogate. 
%it is a necessary condition that a hinge loss be an extension of a possibly rescaled asymmetric loss for consistent estimation in the binary setting~\cite{pre06166984}.  This condition therefore carries over to the more general setting considered here in which $\Delta$ is a set function.

\subsection{Set Functions and Submodularity}
For many optimization problems, a function defined on the power set
 of a given base set $V=\{1,\cdots,p\}$ ($p=|V|$), %\footnote{For notational convenience, we identify each element of the power set $\mathcal{P}(V)$ with a binary indicator vector.} 
a \textit{set function} is often taken into consideration to be minimized (or maximized). Submodular functions play an important role among these set functions, similar to convex functions on vector spaces. 
%, as many functions that occur in practical problems turn out to be submodular functions, and the submodularity may help to determine the links of combinatorial optimization problems.

Submodular functions may be defined through several equivalent properties.  We use the following definition~\cite{fujishige2005submodular}:
\begin{defin}\label{def:submodular}
A set function $l:\mathcal{P}(V)\mapsto\mathbb{R}$ is \textbf{submodular} if and only if for all subsets $A,B\subseteq V$,
\begin{equation}
 l(A)+l(B)\geq l(A\cup B)+l(A\cap B).
\end{equation}
An equivalent definition known as the diminishing returns property follows: for all $B\subseteq A \subset V$ and $x \in V \setminus B$
\begin{equation}\label{eq:SubmodularityDimRet}
    l(B \cup \{x\}) - l(B) \geq l(A \cup \{x\}) - l(A)
  \end{equation}
\end{defin}
A function is \emph{supermodular} iff its negative is submodular, and a function is modular iff it is both submodular and supermodular.  A modular function can be written as a dot product between a binary vector in $\{0,1\}^p$ encoding a subset of $V$ and a coefficient vector in $\mathbb{R}^p$ which uniquely identifies the modular function.  By example, Hamming loss is a modular function with a coefficient vector of all ones, and a subset defined by the entries that differ between two vectors.

Necessary to the sequel is the notion of monotone set functions
\begin{defin}
A set function $l:\mathcal{P}(V)\mapsto\mathbb{R}$ is \textbf{increasing} if and only if for all subsets $A\subset V$ and elements $x \in V \setminus A$, 
\begin{equation}
l(A) \leq l(A \cup \{x\}).
\end{equation}
\end{defin}
In this paper, we consider loss functions for multiple outputs that are set functions where inclusion in a set is defined by a corresponding prediction being incorrect:
\begin{equation}\label{eq:delta_l}
\Delta(y,\tilde{y}) = l(\{i | y^i \neq \tilde{y}^i\}) 
\end{equation}
for some set function $l$. 
Such functions are typically increasing, though it is possible to conceive of a sensible loss function that may be non-increasing.

With these notions, we now turn to an analysis of margin and slack rescaling, and show necessary and sufficient conditions for these operators to yield an extension to the underlying discrete loss function.


==> jaccardlossArXiv.tex <==
\section{Jaccard Loss}\label{sec:jaccard}
The Jaccard index score is a popular measure for comparing the similarity between two sample sets, widely applied in diverse prediction problems such as structured output prediction~\cite{BlaschkoECCV2008}, social network prediction~\cite{liben2007link} and image segmentation~\cite{unnikrishnan2007toward}.  It is used in the evaluation of popular computer vision challenges, such as PASCAL VOC~\cite{pascal-voc-2007} and ImageNet~\cite[Sec.~4.2]{DBLP:journals/corr/RussakovskyDSKSMHKKBBF14}. In this section, we introduce the Jaccard loss based on the Jaccard index score, and we prove that the Jaccard loss is a submodular function with respect to the set of mispredicted elements.

We will use $P_{y},P_{\tilde{y}} \subseteq V$ to denote sets of positive predictions.  We define the Jaccard loss to be~\cite{BlaschkoECCV2008}
\begin{equation}
  \Delta_{J}(y,\tilde{y}) := 1 - \frac{|P_{y}\cap P_{\tilde{y}}|}{|P_{y} \cup P_{\tilde{y}}|}\label{eq:jaccard}
\end{equation}
We now show that this is submodular under the isomorphism $(y,\tilde{y}) \rightarrow A := \{i | y_i \neq \tilde{y}_i\}$, $\Delta_{J}(y,\tilde{y}) \cong l(A)$.  We will use the diminishing returns definition of submodularity as in Definition~\ref{def:submodular}.
We will denote $m := |P_{y}| > 0$, $p := | P_{\tilde{y}} \setminus P_{y} |$, and $n := | P_{y} \setminus P_{\tilde{y}} |$.
With this notation, we have that
\begin{equation}
  \Delta_{J}(y,\tilde{y}) = 1 - \frac{m-n}{m+p}
\end{equation}
For a fixed groundtruth $y$, we have for two sets of mispredictions $A$ and $B$
\begin{equation}
\text{if } B\subseteq A \text{,  then }\  n_B \leq n_A,\  p_B\leq p_A
\end{equation}
We first prove two lemmas about the submodularity of the loss function restricted to additional false positives or false negatives.
\begin{lem}\label{lem:fnSupermodular}
  $\Delta_J$ restricted to marginal false negatives is submodular.
\end{lem}
\begin{proof}
If $i$ is an extra false negative, 
\begin{align}
\Delta_J(A\cup\{i\}) & = \Delta_J(n_A+1,p_A)\nonumber \\
& = \frac{n_A+p_A+1}{m+p_A} \nonumber\\
& = \Delta_J(A) + \frac{1}{m+p_A}
\end{align}
Then we have
\begin{align}
\Delta_J(A\cup\{i\}) - \Delta_J(A) & =  \frac{1}{m+p_A} \nonumber\\
& \leq \frac{1}{m+p_B} \nonumber\\
& = \Delta_J(B\cup\{i\})-\Delta_J(B) 
\end{align}
which complies with the definition of submodularity.
\end{proof}

\begin{lem}\label{lem:JaccardSubFP}
  $\Delta_J$ restricted to marginal false positives is submodular.
\end{lem}
\begin{proof}
If $i$ is an extra false positive, with the similar procedure as previous, we have
\begin{align}
\Delta_J(A\cup\{i\}) & = \Delta_J(n_A,p_A+1) \nonumber\\
& = \frac{n_A+p_A+1}{m+p_A+1}  \\
\Delta_J(A\cup\{i\}) - \Delta_J(A) & = \frac{n_A+p_A+1}{m+p_A+1} - \frac{n_A+p_A}{m+p_A} \nonumber \\
& =  \frac{|A|-n_A}{(m+p_A+1)(m+p_A)} \nonumber\\
& \leq \frac{|A|-n_B}{(m+p_B+1)(m+p_B)} \nonumber\\
& = \Delta_J(B\cup\{i\})-\Delta_J(B)  
\end{align} 
which also complies with the definition of submodularity.
\end{proof}

\begin{pro}
$\Delta_J$ is submodular w.r.t.\ the set of misprediction .
\end{pro}
\begin{proof}
  Lemmas~\ref{lem:fnSupermodular} and~\ref{lem:JaccardSubFP} cover mutually exclusive cases whose union covers all possible marginal mistakes.  As the diminishing returns property of submodularity (Equation~\eqref{eq:SubmodularityDimRet}) holds in both cases, it also holds for the union.
\end{proof}

